A Comprehensive Study on Learning-Based PE Malware Family Classification Methods

Driven by the high profit, Portable Executable (PE) malware has been consistently evolving in terms of both volume and sophistication. PE malware family classification has gained great attention and a large number of approaches have been proposed. With the rapid development of machine learning techniques and the exciting results they achieved on various tasks, machine learning algorithms have also gained popularity in the PE malware family classification task. Three mainstream approaches that use learning based algorithms, as categorized by the input format the methods take, are image-based, binary-based and disassembly-based approaches. Although a large number of approaches are published, there is no consistent comparisons on those approaches, especially from the practical industry adoption perspective. Moreover, there is no comparison in the scenario of concept drift, which is a fact for the malware classification task due to the fast evolving nature of malware. In this work, we conduct a thorough empirical study on learning-based PE malware classification approaches on 4 different datasets and consistent experiment settings. Based on the experiment results and an interview with our industry partners, we find that (1) there is no individual class of methods that significantly outperforms the others; (2) All classes of methods show performance degradation on concept drift (by an average F1-score of 32.23%); and (3) the prediction time and high memory consumption hinder existing approaches from being adopted for industry usage.

==> tab_result_BIG-15.tex <==
\begin{table*}[t]
\centering\footnotesize
\begin{threeparttable}
\caption{Performance Comparison on BIG-15 Dataset (10-fold cross-validation)}
\label{tab:BIG15}
\begin{tabular}{c|c|c|cccc|c|ccc}
\toprule
\hline
\multirow{2}{*}{\textbf{Category}} & \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Training Strategy}} & \multicolumn{4}{c|}{\textbf{Classification Performance (\%)}}     & \multirow{2}{*}{\textbf{Train Time (min)}} & \multicolumn{3}{c}{\textbf{Resource Overhead}}                                                          \\ \cline{4-7} \cline{9-11} 
                                   &                                 &                                             & \textbf{$A$}     & \textbf{$P_{macro}$}     & \textbf{$R_{macro}$}     & \textbf{$F1_{macro}$}    &                                            & \multicolumn{1}{c|}{\textbf{Mem (GB)}} & \multicolumn{1}{c|}{\textbf{GPU.Mem (GB)}} & \textbf{GPU (\%)} \\ \hline
\multirow{20}{*}{Image}            & \multirow{5}{*}{ResNet-50}      & From Scratch                                & \textbf{98.42} & \textbf{96.57} & \textbf{95.68} & \textbf{96.08} & 60.13                                      & \multicolumn{1}{c|}{36.86}              & \multicolumn{1}{c|}{10.77}                 & 85                \\
                                   &                                 & 10\% TL                                     & 94.76          & 92.74          & 82.69          & 86.77          & 3.97                                       & \multicolumn{1}{c|}{22.53}              & \multicolumn{1}{c|}{10.56}                 & 3                 \\
                                   &                                 & 50\% TL                                     & 96.68          & 95.35          & 85.22          & 91.50          & 24.78                                      & \multicolumn{1}{c|}{22.53}              & \multicolumn{1}{c|}{10.56}                 & 3                 \\
                                   &                                 & 80\% TL                                     & 96.90          & 94.87          & 85.53          & 92.50          & 37.02                                      & \multicolumn{1}{c|}{23.55}              & \multicolumn{1}{c|}{10.56}                 & 3                 \\
                                   &                                 & 100\% TL                                    & 97.05          & 95.64          & 93.60          & 94.48          & 43.62                                      & \multicolumn{1}{c|}{21.50}              & \multicolumn{1}{c|}{10.56}                 & 4                 \\ \cline{2-11} 
                                   & \multirow{5}{*}{VGG-16}         & From Scratch                                & 93.94          & 90.32          & 81.89          & 87.28          & 275.52                                     & \multicolumn{1}{c|}{27.65}              & \multicolumn{1}{c|}{10.90}                 & 75                \\
                                   &                                 & 10\% TL                                     & 89.56          & 78.74          & 76.73          & 77.59          & 0.42                                       & \multicolumn{1}{c|}{19.46}              & \multicolumn{1}{c|}{10.44}                 & 3                 \\
                                   &                                 & 50\% TL                                     & 95.21          & 89.02          & 83.77          & 87.21          & 11.76                                      & \multicolumn{1}{c|}{21.50}              & \multicolumn{1}{c|}{10.44}                 & 44                \\
                                   &                                 & 80\% TL                                     & 96.62          & 92.00          & 85.20          & 90.41          & 8.04                                       & \multicolumn{1}{c|}{22.53}              & \multicolumn{1}{c|}{10.44}                 & 71                \\
                                   &                                 & 100\% TL                                    & \textbf{96.78} & \textbf{93.36} & \textbf{91.78} & \textbf{92.46} & 9.72                                       & \multicolumn{1}{c|}{23.55}              & \multicolumn{1}{c|}{10.44}                 & 70                \\ \cline{2-11} 
                                   & \multirow{5}{*}{Inception-V3}   & From Scratch                                & \textbf{96.99} & \textbf{93.67} & \textbf{94.46} & \textbf{94.03} & 120                                        & \multicolumn{1}{c|}{36.86}              & \multicolumn{1}{c|}{10.77}                 & 71                \\
                                   &                                 & 10\% TL                                     & 92.28          & 91.46          & 80.51          & 80.94          & 3.27                                       & \multicolumn{1}{c|}{18.43}              & \multicolumn{1}{c|}{10.56}                 & 4                 \\
                                   &                                 & 50\% TL                                     & 95.10          & 91.17          & 86.76          & 86.87          & 12.78                                      & \multicolumn{1}{c|}{19.46}              & \multicolumn{1}{c|}{10.56}                 & 8                 \\
                                   &                                 & 80\% TL                                     & 95.31          & 92.52          & 88.54          & 88.64          & 19.02                                      & \multicolumn{1}{c|}{19.46}              & \multicolumn{1}{c|}{10.56}                 & 8                 \\
                                   &                                 & 100\% TL                                    & 95.56          & 93.48          & 89.64          & 89.76          & 22.92                                      & \multicolumn{1}{c|}{21.50}              & \multicolumn{1}{c|}{10.56}                 & 17                \\ \cline{2-11} 
                                   & \multirow{5}{*}{IMCFN}          & From Scratch                                & 97.77          & 95.93          & 94.81          & 95.13          & 52.32                                      & \multicolumn{1}{c|}{58.37}              & \multicolumn{1}{c|}{10.77}                 & 95                \\
                                   &                                 & 10\% TL                                     & 94.81          & 94.13          & 84.04          & 85.21          & 4.52                                       & \multicolumn{1}{c|}{20.48}              & \multicolumn{1}{c|}{10.44}                 & 25                \\
                                   &                                 & 50\% TL                                     & 97.38          & 95.25          & 91.90          & 93.15          & 14.13                                      & \multicolumn{1}{c|}{22.53}              & \multicolumn{1}{c|}{10.44}                 & 34                \\
                                   &                                 & 80\% TL                                     & 97.81          & 96.09          & 93.69          & 94.69          & 21.04                                      & \multicolumn{1}{c|}{28.67}              & \multicolumn{1}{c|}{10.44}                 & 40                \\
                                   &                                 & 100\% TL                                    & \textbf{98.05} & \textbf{96.18} & \textbf{94.37} & \textbf{95.18} & 21.41                                      & \multicolumn{1}{c|}{32.77}              & \multicolumn{1}{c|}{10.44}                 & 40                \\ \hline
\multirow{2}{*}{Binary}            & CBOW+MLP                        & -                                           & \textbf{98.41} & \textbf{97.63} & \textbf{96.67} & \textbf{97.12} & 1.46                                       & \multicolumn{1}{c|}{13.31}              & \multicolumn{1}{c|}{10.44}                 & 29                \\
                                   & MalConv                         & -                                           & 97.02          & 94.34          & 92.62          & 93.33          & 227.40                                     & \multicolumn{1}{c|}{259.07}             & \multicolumn{1}{c|}{10.79$\times$4}               & 37                \\ \hline
\multirow{3}{*}{Disassembly}       & MAGIC                           & -                                           & 98.05          & \textbf{96.75} & 94.03          & 95.14          & 52.32                                      & \multicolumn{1}{c|}{13.31}              & \multicolumn{1}{c|}{9.88}                  & 73                \\
                                   & Word2Vec+KNN                    & -                                           & \textbf{98.07} & 96.41          & \textbf{96.51} & \textbf{96.45} & 0.09                                       & \multicolumn{1}{c|}{1.30}               & \multicolumn{1}{c|}{-}                     & -                 \\
                                   & MCSC                            & -                                           & 97.94          & 95.97          & 96.17          & 96.06          & 3.62                                       & \multicolumn{1}{c|}{3.78}               & \multicolumn{1}{c|}{10.77}                 & 33                \\ \hline \bottomrule
\end{tabular}
% \footnotesize
% $^*$ Physical memory; $^{**}$ GPU memory.
\end{threeparttable}
\end{table*}
























\begin{comment}
\begin{table*}[t]
\centering\footnotesize
\begin{threeparttable}
\caption{Comparison of Classification Performance of Various Methods Based on 10-fold Cross-validation on the BIG-15 Dataset}
\label{tab:BIG15-11}
\begin{tabular}{c|c|c|cccc|c|ccc}
\toprule
\hline
                                    &                                  &                                              & \multicolumn{4}{c|}{\textbf{Classification Performance (\%)}}                                                             &                                             & \multicolumn{3}{c}{\textbf{Reasource Overhead}}                                                                                   \\ \cline{4-7} \cline{9-11} 
\multirow{-2}{*}{\textbf{Category}} & \multirow{-2}{*}{\textbf{Model}} & \multirow{-2}{*}{\textbf{Training Strategy}} & \textbf{A}                   & \textbf{P}                   & \textbf{R}                   & \textbf{F1}                  & \multirow{-2}{*}{\textbf{Train Time (min)}} & \multicolumn{1}{c|}{\textbf{Mem* (GB)}}           & \multicolumn{1}{c|}{\textbf{G.Mem** (GB)}}        & \textbf{GPU (\%)}         \\ \hline
                                    &                                  & From Scratch                                 & \textbf{98.42}               & \textbf{96.57}               & \textbf{95.68}               & \textbf{96.08}               & 60.13                                       & \multicolumn{1}{c|}{36.86}                        & \multicolumn{1}{c|}{10.77}                        & 85                        \\
                                    &                                  & 10\% TL                                      & 94.76                        & 92.74                        & 82.69                        & 86.77                        & 3.97                                        & \multicolumn{1}{c|}{22.53}                        & \multicolumn{1}{c|}{10.56}                        & 3                         \\
                                    &                                  & 50\% TL                                      & 96.68                        & 95.35                        & 85.22                        & 91.50                        & 24.78                                       & \multicolumn{1}{c|}{22.53}                        & \multicolumn{1}{c|}{10.56}                        & 3                         \\
                                    &                                  & 80\% TL                                      & 96.90                        & 94.87                        & 85.53                        & 92.50                        & 37.02                                       & \multicolumn{1}{c|}{23.55}                        & \multicolumn{1}{c|}{10.56}                        & 3                         \\
                                    & \multirow{-5}{*}{ResNet-50}      & 100\% TL                                     & 97.05                        & 95.64                        & 93.60                        & 94.48                        & 43.62                                       & \multicolumn{1}{c|}{21.50}                        & \multicolumn{1}{c|}{10.56}                        & 4                         \\ \cline{2-11} 
                                    &                                  & From Scratch                                 & 93.94                        & 90.32                        & 81.89                        & 87.28                        & 275.52                                      & \multicolumn{1}{c|}{27.65}                        & \multicolumn{1}{c|}{10.90}                        & 75                        \\
                                    &                                  & 10\% TL                                      & 89.56                        & 78.74                        & 76.73                        & 77.59                        & 0.42                                        & \multicolumn{1}{c|}{19.46}                        & \multicolumn{1}{c|}{10.44}                        & 3                         \\
                                    &                                  & 50\% TL                                      & 95.21                        & 89.02                        & 83.77                        & 87.21                        & 11.76                                       & \multicolumn{1}{c|}{21.50}                        & \multicolumn{1}{c|}{10.44}                        & 44                        \\
                                    &                                  & 80\% TL                                      & 96.62                        & 92.00                        & 85.20                        & 90.41                        & 8.04                                        & \multicolumn{1}{c|}{22.53}                        & \multicolumn{1}{c|}{10.44}                        & 71                        \\
                                    & \multirow{-5}{*}{VGG-16}         & 100\% TL                                     & \textbf{96.78}               & \textbf{93.36}               & \textbf{91.78}               & \textbf{92.46}               & 9.72                                        & \multicolumn{1}{c|}{23.55}                        & \multicolumn{1}{c|}{10.44}                        & 70                        \\ \cline{2-11} 
                                    &                                  & From Scratch                                 & \textbf{96.99}               & \textbf{93.67}               & \textbf{94.46}               & \textbf{94.03}               & 120                                         & \multicolumn{1}{c|}{36.86}                        & \multicolumn{1}{c|}{10.77}                        & 71                        \\
                                    &                                  & 10\% TL                                      & 92.28                        & 91.46                        & 80.51                        & 80.94                        & 3.27                                        & \multicolumn{1}{c|}{18.43}                        & \multicolumn{1}{c|}{10.56}                        & 4                         \\
                                    &                                  & 50\% TL                                      & 95.10                        & 91.17                        & 86.76                        & 86.87                        & 12.78                                       & \multicolumn{1}{c|}{19.46}                        & \multicolumn{1}{c|}{10.56}                        & 8                         \\
                                    &                                  & 80\% TL                                      & 95.31                        & 92.52                        & 88.54                        & 88.64                        & 19.02                                       & \multicolumn{1}{c|}{19.46}                        & \multicolumn{1}{c|}{10.56}                        & 8                         \\
                                    & \multirow{-5}{*}{Inception-V3}   & 100\% TL                                     & 95.56                        & 93.48                        & 89.64                        & 89.76                        & 22.92                                       & \multicolumn{1}{c|}{21.50}                        & \multicolumn{1}{c|}{10.56}                        & 17                        \\ \cline{2-11} 
                                    &                                  & From Scratch                                 & 97.77                        & 95.93                        & 94.81                        & 95.13                        & 52.32                                       & \multicolumn{1}{c|}{58.37}                        & \multicolumn{1}{c|}{10.77}                        & 95                        \\ \cline{3-11} 
                                    &                                  & {\color[HTML]{FE0000} 10\% TL}               & {\color[HTML]{FE0000} 94.81} & {\color[HTML]{FE0000} 94.13} & {\color[HTML]{FE0000} 84.04} & {\color[HTML]{FE0000} 85.21} & {\color[HTML]{FE0000} 4.52}                 & \multicolumn{1}{c|}{{\color[HTML]{FE0000} 20.48}} & \multicolumn{1}{c|}{{\color[HTML]{FE0000} 10.44}} & {\color[HTML]{FE0000} 25} \\
                                    &                                  & {\color[HTML]{FE0000} 50\% TL}               & {\color[HTML]{FE0000} 97.38} & {\color[HTML]{FE0000} 95.25} & {\color[HTML]{FE0000} 91.90} & {\color[HTML]{FE0000} 93.15} & {\color[HTML]{FE0000} 14.13}                & \multicolumn{1}{c|}{{\color[HTML]{FE0000} 22.53}} & \multicolumn{1}{c|}{{\color[HTML]{FE0000} 10.44}} & {\color[HTML]{FE0000} 34} \\
                                    &                                  & {\color[HTML]{FE0000} 80\% TL}               & {\color[HTML]{FE0000} 97.81} & {\color[HTML]{FE0000} 96.09} & {\color[HTML]{FE0000} 93.69} & {\color[HTML]{FE0000} 94.69} & {\color[HTML]{FE0000} 21.04}                & \multicolumn{1}{c|}{{\color[HTML]{FE0000} 28.67}} & \multicolumn{1}{c|}{{\color[HTML]{FE0000} 10.44}} & {\color[HTML]{FE0000} 40} \\
                                    &                                  & {\color[HTML]{FE0000} 100\% TL}              & {\color[HTML]{FE0000} 98.05} & {\color[HTML]{FE0000} 96.18} & {\color[HTML]{FE0000} 94.37} & {\color[HTML]{FE0000} 95.18} & {\color[HTML]{FE0000} 21.41}                & \multicolumn{1}{c|}{{\color[HTML]{FE0000} 32.77}} & \multicolumn{1}{c|}{{\color[HTML]{FE0000} 10.44}} & {\color[HTML]{FE0000} 40} \\ \cline{3-11} 
                                    &                                  & 10\% TL                                      & 94.80                        & 89.05                        & 82.76                        & 83.77                        & 10.06                                       & \multicolumn{1}{c|}{38.91}                        & \multicolumn{1}{c|}{10.77}                        & 73                        \\
                                    &                                  & 50\% TL                                      & 97.93                        & 95.43                        & 86.67                        & 93.64                        & 24.63                                       & \multicolumn{1}{c|}{54.27}                        & \multicolumn{1}{c|}{10.77}                        & 89                        \\
                                    &                                  & 80\% TL                                      & 98.48                        & 96.90                        & 87.31                        & 95.38                        & 68.96                                       & \multicolumn{1}{c|}{56.32}                        & \multicolumn{1}{c|}{10.77}                        & 89                        \\
\multirow{-24}{*}{Image}            & \multirow{-9}{*}{IMCFN}          & 100\% TL                                     & \textbf{99.17}               & \textbf{98.69}               & \textbf{97.52}               & \textbf{98.07}               & 46.00                                       & \multicolumn{1}{c|}{58.37}                        & \multicolumn{1}{c|}{10.77}                        & 88                        \\ \hline
                                    & CBOW+MLP                         & -                                            & \textbf{98.41}               & \textbf{97.63}               & \textbf{96.67}               & \textbf{97.12}               & 1.46                                        & \multicolumn{1}{c|}{13.31}                        & \multicolumn{1}{c|}{10.44}                        & 29                      \\
\multirow{-2}{*}{Binary}            & MalConv                          & -                                            & 97.02                        & 94.34                        & 92.62                        & 93.33                        & 227.40                                      & \multicolumn{1}{c|}{259.07}                       & \multicolumn{1}{c|}{10.79*4}                      & 37                      \\ \hline
                                    & MAGIC                            & -                                            & 98.05                        & \textbf{96.75}               & 94.03                        & 95.14                        & 52.32                                       & \multicolumn{1}{c|}{13.31}                        & \multicolumn{1}{c|}{9.88}                         & 73                      \\
                                    & Word2Vec+KNN                     & -                                            & \textbf{98.07}               & 96.41                        & \textbf{96.51}               & \textbf{96.45}               & 0.09                                        & \multicolumn{1}{c|}{1.30}                         & \multicolumn{1}{c|}{-}                            & -                         \\
\multirow{-3}{*}{Disassembly}       & MCSC                             & -                                            & 97.94                        & 95.97                        & 96.17                        & 96.06                        & 3.62                                        & \multicolumn{1}{c|}{3.78}                         & \multicolumn{1}{c|}{10.77}                        & 33                      \\ \hline
\bottomrule
\end{tabular}
\footnotesize
$^*$ Physical memory; $^{**}$ GPU memory.
~\\
\yx{red data: IMCFN doesn't open the last feature extraction block (setting is consistent with other models). 
~\\
black data: IMCFN open the last feature extraction block.
~\\
BIG-15 dataset is imbalanced.}
\end{threeparttable}
\end{table*}
\end{comment}








\begin{comment}
\begin{table*}[t]
\centering\scriptsize
\begin{threeparttable}
\caption{Comparison of Classification Performance of Various Methods Based on 10-fold Cross-validation on the BIG-15 Dataset}
\label{tab:BIG15-2}
\begin{tabular}{c|c|c|cccc|c|ccc}
\toprule
\hline
\multirow{2}{*}{\textbf{Category}} & \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Training Strategy}} & \multicolumn{4}{c|}{\textbf{Classification Performance (\%)}}     & \multirow{2}{*}{\textbf{Train Time (min)}} & \multicolumn{3}{c}{\textbf{Resource Overhead}}                                                           \\ \cline{4-7} \cline{9-11} 
                                   &                                 &                                             & \textbf{A}     & \textbf{P}     & \textbf{R}     & \textbf{F1}    &                                            & \multicolumn{1}{c|}{\textbf{Mem* (GB)}} & \multicolumn{1}{c|}{\textbf{G.Mem** (MiB)}} & \textbf{GPU (\%)} \\ \hline
\multirow{20}{*}{Image}            & \multirow{5}{*}{ResNet-50}      & From Scratch                                & \textbf{98.42} & \textbf{96.57} & \textbf{95.68} & \textbf{96.08} & 60.13                                      & \multicolumn{1}{c|}{36.86}              & \multicolumn{1}{c|}{10.77}                  & 85                \\
                                   &                                 & 10\% TL                                     & 94.76          & 92.74          & 82.69          & 86.77          & 3.97                                       & \multicolumn{1}{c|}{22.53}              & \multicolumn{1}{c|}{10.56}                  & 3                 \\
                                   &                                 & 50\% TL                                     & 96.68          & 95.35          & 85.22          & 91.50          & 24.78                                      & \multicolumn{1}{c|}{22.53}              & \multicolumn{1}{c|}{10.56}                  & 3                 \\
                                   &                                 & 80\% TL                                     & 96.90          & 94.87          & 85.53          & 92.50          & 37.02                                      & \multicolumn{1}{c|}{23.55}              & \multicolumn{1}{c|}{10.56}                  & 3                 \\
                                   &                                 & 100\% TL                                    & 97.05          & 95.64          & 93.60          & 94.48          & 43.62                                      & \multicolumn{1}{c|}{21.50}              & \multicolumn{1}{c|}{10.56}                  & 4                 \\ \cline{2-11} 
                                   & \multirow{5}{*}{VGG-16}         & From Scratch                                & 93.94          & 90.32          & 81.89          & 87.28          & 275.52                                     & \multicolumn{1}{c|}{27.65}              & \multicolumn{1}{c|}{10.77}                  & 75                \\
                                   &                                 & 10\% TL                                     & 89.56          & 78.74          & 76.73          & 77.59          & 0.42                                       & \multicolumn{1}{c|}{19.46}              & \multicolumn{1}{c|}{10.44}                  & 3                 \\
                                   &                                 & 50\% TL                                     & 95.21          & 89.02          & 83.77          & 87.21          & 11.76                                      & \multicolumn{1}{c|}{21.50}              & \multicolumn{1}{c|}{10.44}                  & 44                \\
                                   &                                 & 80\% TL                                     & 96.62          & 92.00          & 85.20          & 90.41          & 8.04                                       & \multicolumn{1}{c|}{22.53}              & \multicolumn{1}{c|}{10.44}                  & 71                \\
                                   &                                 & 100\% TL                                    & \textbf{96.78} & \textbf{93.36} & \textbf{91.78} & \textbf{92.46} & 9.72                                       & \multicolumn{1}{c|}{23.55}              & \multicolumn{1}{c|}{10.44}                  & 70                \\ \cline{2-11} 
                                   & \multirow{5}{*}{Inception-V3}   & From Scratch                                & \textbf{96.99} & \textbf{93.67} & \textbf{94.46} & \textbf{94.03} & 120                                        & \multicolumn{1}{c|}{36.86}              & \multicolumn{1}{c|}{10.77}                  & 71                \\
                                   &                                 & 10\% TL                                     & 92.28          & 91.46          & 80.51          & 80.94          & 3.27                                       & \multicolumn{1}{c|}{18.43}              & \multicolumn{1}{c|}{10.56}                  & 4                 \\
                                   &                                 & 50\% TL                                     & 95.10          & 91.17          & 86.76          & 86.87          & 12.78                                      & \multicolumn{1}{c|}{19.46}              & \multicolumn{1}{c|}{10.56}                  & 8                 \\
                                   &                                 & 80\% TL                                     & 95.31          & 92.52          & 88.54          & 88.64          & 19.02                                      & \multicolumn{1}{c|}{19.46}              & \multicolumn{1}{c|}{10.56}                  & 8                 \\
                                   &                                 & 100\% TL                                    & 95.56          & 93.48          & 89.64          & 89.76          & 22.92                                      & \multicolumn{1}{c|}{21.50}              & \multicolumn{1}{c|}{10.56}                  & 17                \\ \cline{2-11} 
                                   & \multirow{5}{*}{IMCFN}          & From Scratch                                & 97.77          & 95.93          & 94.81          & 95.13          & 52.32                                      & \multicolumn{1}{c|}{58.37}              & \multicolumn{1}{c|}{10.77}                  & 95                \\
                                   &                                 & 10\% TL                                     & 94.80          & 89.05          & 82.76          & 83.77          & 10.06                                      & \multicolumn{1}{c|}{38.91}              & \multicolumn{1}{c|}{10.77}                  & 73                \\
                                   &                                 & 50\% TL                                     & 97.93          & 95.43          & 86.67          & 93.64          & 24.63                                      & \multicolumn{1}{c|}{54.27}              & \multicolumn{1}{c|}{10.77}                  & 89                \\
                                   &                                 & 80\% TL                                     & 98.48          & 96.90          & 87.31          & 95.38          & 68.96                                      & \multicolumn{1}{c|}{56.32}              & \multicolumn{1}{c|}{10.77}                  & 89                \\
                                   &                                 & 100\% TL                                    & \textbf{99.17} & \textbf{98.69} & \textbf{97.52} & \textbf{98.07(\yx{91.41$^\star$})} & 46.00                                      & \multicolumn{1}{c|}{58.37}              & \multicolumn{1}{c|}{10.77}                  & 88                \\ \hline
\multirow{2}{*}{Binary}            & CBOW+MLP                        & -                                           & \textbf{98.41} & \textbf{97.63} & \textbf{96.67} & \textbf{97.12} & 1.46                                       & \multicolumn{1}{c|}{13.31}              & \multicolumn{1}{c|}{10.44}                  & 29\%              \\
                                   & MalConv                         & -                                           & 97.02          & 94.34          & 92.62          & 93.33          & 227.40                                     & \multicolumn{1}{c|}{259.07}             & \multicolumn{1}{c|}{10.79$\times$4}          & 37\%              \\ \hline
\multirow{3}{*}{Disassembly}       & MAGIC                           & -                                           & 98.05          & \textbf{96.75} & 94.03          & 95.14          & 52.32                                      & \multicolumn{1}{c|}{13.31}              & \multicolumn{1}{c|}{9.88}                   & 73\%              \\
                                   & Word2Vec+KNN                    & -                                           & \textbf{98.07} & 96.41          & \textbf{96.51} & \textbf{96.45} & 0.09                                       & \multicolumn{1}{c|}{1.30}               & \multicolumn{1}{c|}{-}                      & -                 \\
                                   & MCSC                            & -                                           & 97.94          & 95.97          & 96.17          & 96.06          & 3.62                                       & \multicolumn{1}{c|}{3.78}               & \multicolumn{1}{c|}{10.77}                  & 33\%              \\ \hline
\bottomrule
\end{tabular}
\footnotesize
$^*$ Physical memory; $^{**}$ GPU memory.
~\\
\yx{$^\star$ IMCFN doesn't open the last feature extraction block (setting is consistent with other models). IMCFN is not the best in 100\% TL compared with other models.
~\\
BIG-15 dataset is imbalanced.}
%\begin{tablenotes}
% \item[*]  Physical memory
% \item[**] GPU memory
% \item[***] 4 GPUs are used
%\item[3] Time: The time includes data pre-processing time and model training time. The data preparation time is average time for processing a sample, and for each method is composed as follows. IMCFN: the time taken to convert a malware sample to a 224*224 size color image; CBOW+MLP: the time to delete the useless bytes from a binary file, and the time to convert the processed file to a 256*256 dimensional ascending vector matrix; MalConv: The time to process a binary file to a 2MB size; MAGIC: The time to extract an ACFG; Word2Vec+KNN: The time to parse a disassembly file into Opcode sequences, and the time to calculate the document distance between a test sample and all training samples; MCSC: The time to extract the Opcode sequence from a disassembly file and convert it to an image based on Simhash. \jj{Move to configuration part if necessary?}
%\end{tablenotes}
\end{threeparttable}
\end{table*}
\end{comment}













\begin{comment}
\begin{table*}[t]
\centering\scriptsize
\begin{threeparttable}
\caption{Comparison of Classification Performance of Various Methods Based on 10-fold Cross-validation on the BIG-15 Dataset}
\label{tab:Compare-BIG-15-early stop epoch}
\begin{tabular}{c|c|c|cccc|c|c|ccl}
\toprule
\hline
\multirow{2}{*}{\textbf{Category}} & \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Training Strategy}} & \multicolumn{4}{c|}{\textbf{Classification Performance (\%)}}     & \multicolumn{2}{c|}{\textbf{Time}}           & \multicolumn{3}{c}{\textbf{Reasource Overhead}}                                                                        \\ \cline{4-12} 
                                   &                                 &                                             & \textbf{A}     & \textbf{P}     & \textbf{R}     & \textbf{F1}    & \textbf{Pre (s)}      & \textbf{Train (min)} & \multicolumn{1}{c|}{\textbf{V.Mem (GB)}} & \multicolumn{1}{c|}{\textbf{G.Mem (GB)}} & \multicolumn{1}{c}{\textbf{GPU}} \\ \hline
\multirow{20}{*}{Image}            & \multirow{5}{*}{ResNet-50}      & From Scratch                                & \textbf{98.42} & \textbf{96.57} & \textbf{95.68} & \textbf{96.08} & \multirow{20}{*}{0.7} & 60.13                & \multicolumn{1}{c|}{}                    & \multicolumn{1}{c|}{}                    &                                  \\
                                   &                                 & 10\%-Transfer                               & 94.76          & 92.74          & 82.69          & 86.77          &                       & 3.97                 & \multicolumn{1}{c|}{}                    & \multicolumn{1}{c|}{}                    &                                  \\
                                   &                                 & 50\%-Transfer                               & 96.68          & 95.35          & 85.22          & 91.50          &                       & 24.78                & \multicolumn{1}{c|}{}                    & \multicolumn{1}{c|}{}                    &                                  \\
                                   &                                 & 80\%-Transfer                               & 96.90          & 94.87          & 85.53          & 92.50          &                       & 37.02                & \multicolumn{1}{c|}{}                    & \multicolumn{1}{c|}{}                    &                                  \\
                                   &                                 & 100\%-Transfer                              & 97.05          & 95.64          & 93.60          & 94.48          &                       & 43.62                & \multicolumn{1}{c|}{}                    & \multicolumn{1}{c|}{}                    &                                  \\ \cline{2-7} \cline{9-12} 
                                   & \multirow{5}{*}{VGG-16}         & From Scratch                                & 93.94          & 90.32          & 81.89          & 87.28          &                       & 275.52               & \multicolumn{1}{c|}{}                    & \multicolumn{1}{c|}{}                    &                                  \\
                                   &                                 & 10\%-Transfer                               & 89.56          & 78.74          & 76.73          & 77.59          &                       & 0.42                 & \multicolumn{1}{c|}{}                    & \multicolumn{1}{c|}{}                    &                                  \\
                                   &                                 & 50\%-Transfer                               & 95.21          & 89.02          & 83.77          & 87.21          &                       & 11.76                & \multicolumn{1}{c|}{}                    & \multicolumn{1}{c|}{}                    &                                  \\
                                   &                                 & 80\%-Transfer                               & 96.62          & 92.00          & 85.20          & 90.41          &                       & 8.04                 & \multicolumn{1}{c|}{}                    & \multicolumn{1}{c|}{}                    &                                  \\
                                   &                                 & 100\%-Transfer                              & \textbf{96.78} & \textbf{93.36} & \textbf{91.78} & \textbf{92.46} &                       & 9.72                 & \multicolumn{1}{c|}{}                    & \multicolumn{1}{c|}{}                    &                                  \\ \cline{2-7} \cline{9-12} 
                                   & \multirow{5}{*}{Inception-V3}   & From Scratch                                & \textbf{96.99} & \textbf{93.67} & \textbf{94.46} & \textbf{94.03} &                       & 120.00                  & \multicolumn{1}{c|}{}                    & \multicolumn{1}{c|}{}                    &                                  \\
                                   &                                 & 10\%-Transfer                               & 92.28          & 91.46          & 80.51          & 80.94          &                       & 3.27                 & \multicolumn{1}{c|}{}                    & \multicolumn{1}{c|}{}                    &                                  \\
                                   &                                 & 50\%-Transfer                               & 95.10          & 91.17          & 86.76          & 86.87          &                       & 12.78                & \multicolumn{1}{c|}{}                    & \multicolumn{1}{c|}{}                    &                                  \\
                                   &                                 & 80\%-Transfer                               & 95.31          & 92.52          & 88.54          & 88.64          &                       & 19.02                & \multicolumn{1}{c|}{}                    & \multicolumn{1}{c|}{}                    &                                  \\
                                   &                                 & 100\%-Transfer                              & 95.56          & 93.48          & 89.64          & 89.76          &                       & 22.92                & \multicolumn{1}{c|}{}                    & \multicolumn{1}{c|}{}                    &                                  \\ \cline{2-7} \cline{9-12} 
                                   & \multirow{5}{*}{IMCFN}          & From Scratch                                & 97.70          & 95.49          & 93.70          & 94.44          &                       & 40.64                & \multicolumn{1}{c|}{}                    & \multicolumn{1}{c|}{}                    &                                  \\
                                   &                                 & 10\%-Transfer                               & 94.80          & 89.05          & 82.76          & 83.77          &                       & 10.06                & \multicolumn{1}{c|}{}                    & \multicolumn{1}{c|}{}                    &                                  \\
                                   &                                 & 50\%-Transfer                               & 97.93          & 95.43          & 86.67          & 93.64          &                       & 24.63                & \multicolumn{1}{c|}{}                    & \multicolumn{1}{c|}{}                    &                                  \\
                                   &                                 & 80\%-Transfer                               & 98.48          & 96.90          & 87.31          & 95.38          &                       & 68.96                & \multicolumn{1}{c|}{}                    & \multicolumn{1}{c|}{}                    &                                  \\
                                   &                                 & 100\%-Transfer                              & \textbf{99.17} & \textbf{98.69} & \textbf{97.52} & \textbf{98.07)} &                       & 46.00                & \multicolumn{1}{c|}{96.14}               & \multicolumn{1}{c|}{10.77}               & \multicolumn{1}{c}{88\%}         \\ \hline
\multirow{2}{*}{Binary}            & CBOW+MLP                        & -                                           & 98.41          & 97.63          & 96.67          & 97.12          & 6.53                  & 1.46                 & \multicolumn{1}{c|}{54.87}               & \multicolumn{1}{c|}{10.44}               & \multicolumn{1}{c}{29\%}         \\
                                   & MalConv                         & -                                           & 97.02          & 94.34          & 92.62          & 93.33          & 0.28                  & 227.40               & \multicolumn{1}{c|}{348.16}              & \multicolumn{1}{c|}{10.79*4}             & \multicolumn{1}{c}{37\%}         \\ \hline
\multirow{3}{*}{Disassembly}       & MAGIC                           & -                                           & 98.05          & 96.75          & 94.03          & 95.14          & 13.87                 & 52.32                & \multicolumn{1}{c|}{42.02}               & \multicolumn{1}{c|}{9.88}                & \multicolumn{1}{c}{73\%}         \\
                                   & Word2Vec+KNN                    & -                                           & 98.07          & 96.41          & 96.51          & 96.45          & 109.14                & 0.09                 & \multicolumn{1}{c|}{6.63}                & \multicolumn{1}{c|}{-}                   & \multicolumn{1}{c}{-}            \\
                                   & MCSC                            & -                                           & 97.94          & 95.97          & 96.17          & 96.06          & 4.06                  & 3.62                 & \multicolumn{1}{c|}{45.12}               & \multicolumn{1}{c|}{10.77}               & \multicolumn{1}{c}{33\%}         \\ \hline
\bottomrule
\end{tabular}
\footnotesize
\begin{tablenotes}
 \item [1] Average Classification Performance: The prediction results of 10-fold are added up into a large confusion matrix, and Accuracy, Precision, Recall and F1-score are then calculated as a whole.
 \item[2] Resource Overhead: The resource includes virtual memory (V.Mem), GPU memory (G.Mem), and GPU-util. The V.Mem of the Word2Vec+KNN method has two values, the first one represent the resource consume for data preparation and the second one is for model training.
 \item[3] Time: The time includes data pre-processing time and model training time. The data preparation time is average time for processing a sample, and for each method is composed as follows. IMCFN: the time taken to convert a malware sample to a 224*224 size color image; CBOW+MLP: the time to delete the useless bytes from a binary file, and the time to convert the processed file to a 256*256 dimensional ascending vector matrix; MalConv: The time to process a binary file to a 2MB size; MAGIC: The time to extract an ACFG; Word2Vec+KNN: The time to parse a disassembly file into Opcode sequences, and the time to calculate the document distance between a test sample and all training samples; MCSC: The time to extract the Opcode sequence from a disassembly file and convert it to an image based on Simhash. \jj{Move to configuration part if necessary?}
\end{tablenotes}
\end{threeparttable}
\end{table*}
\end{comment}














\begin{comment}
\begin{table*}[t]
\centering\scriptsize
\begin{threeparttable}
\caption{Comparison of Classification Performance of Various Methods Based on 10-fold Cross-validation on the BIG-15 Dataset}
\label{tab:Compare-BIG-15-the original epoch}
\begin{tabular}{l|c|c|cccc|c|c|lll}
\toprule
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Category}}} & \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Training Strategy}}  & \multicolumn{4}{c|}{\textbf{Classification Performance (\%)}} & \multicolumn{2}{c|}{\textbf{Time}}                  & \multicolumn{3}{c}{\textbf{Reasource Overhead}}                                                                        \\ \cline{4-12} 
\multicolumn{1}{c|}{}                                   &                                 &                                              & \textbf{A}      & \textbf{P}      & \textbf{R}      & \textbf{F1}     & \textbf{Pre (s)} & \textbf{Train (min)} & \multicolumn{1}{c|}{\textbf{V.Mem (GB)}} & \multicolumn{1}{c|}{\textbf{G.Mem (GB)}} & \multicolumn{1}{c}{\textbf{GPU}} \\ \hline
\multirow{20}{*}{Image}                                 & \multirow{5}{*}{ResNet-50}      & Train From Scretch                           & 98.42           & 96.57           & 95.68           & 96.08           & \multirow{20}{*}{}           & 203.70               & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\
                                                        &                                 & 10\%-Transfer Learning                       & 94.76           & 92.74           & 82.69           & 86.77           &                              & 8.58                 & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\
                                                        &                                 & 50\%-Transfer Learning                       & 96.68           & 95.35           & 85.22           & 91.50           &                              & 24.78                & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\
                                                        &                                 & 80\%-Transfer Learning                       & 96.90           & 94.87           & 85.53           & 92.50           &                              & 37.02                & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\
                                                        &                                 & \multicolumn{1}{l|}{100\%-Transfer Learning} & 97.05           & 95.64           & 93.60           & 94.48           &                              & 43.62                & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\ \cline{2-7} \cline{9-12} 
                                                        & \multirow{5}{*}{VGG-16}         & Train From Scretch                           & 93.94           & 90.32           & 81.89           & 87.28           &                              & 275.52               & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\
                                                        &                                 & 10\%-Transfer Learning                       & 89.56           & 78.74           & 76.73           & 77.59           &                              & 1.52                 & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\
                                                        &                                 & 50\%-Transfer Learning                       & 95.21           & 89.02           & 83.77           & 87.21           &                              & 11.76                & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\
                                                        &                                 & 80\%-Transfer Learning                       & 96.62           & 92.00           & 85.20           & 90.41           &                              & 8.04                 & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\
                                                        &                                 & \multicolumn{1}{l|}{100\%-Transfer Learning} & 96.78           & 93.36           & 91.78           & 92.46           &                              & 9.72                 & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\ \cline{2-7}
                                                        & \multirow{5}{*}{Inception-V3}   & Train From Scretch                           & 96.99           & 93.67           & 94.46           & 94.03           &                              & 150.00               & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\
                                                        &                                 & 10\%-Transfer Learning                       & 92.28           & 91.46           & 80.51           & 80.94           &                              & 4.44                 & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\
                                                        &                                 & 50\%-Transfer Learning                       & 95.10           & 91.17           & 86.76           & 86.87           &                              & 12.78                & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\
                                                        &                                 & 80\%-Transfer Learning                       & 95.31           & 92.52           & 88.54           & 88.64           &                              & 19.02                & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\
                                                        &                                 & \multicolumn{1}{l|}{100\%-Transfer Learning} & 95.56           & 93.48           & 89.64           & 89.76           &                              & 22.92                & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\ \cline{2-7}
                                                        & \multirow{5}{*}{IMCFN}          & Train From Scretch                           & 97.70           & 95.49           & 93.70           & 94.44           &                              & 277.08               & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\
                                                        &                                 & 10\%-Transfer Learning                       & 94.80           & 89.05           & 82.76           & 83.77           &                              & 18.18                & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\
                                                        &                                 & 50\%-Transfer Learning                       & 97.93           & 95.43           & 86.67           & 93.64           &                              & 53.94                & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\
                                                        &                                 & 80\%-Transfer Learning                       & 98.48           & 96.90           & 87.31           & 95.38           &                              & 134.34               & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\
                                                        &                                 & \multicolumn{1}{l|}{100\%-Transfer Learning} & \textbf{99.17}  & \textbf{98.69}  & \textbf{97.52}  & \textbf{98.07}  &                              & 166.68               & \multicolumn{1}{c|}{96.14}               & \multicolumn{1}{c|}{10.77}               & \multicolumn{1}{c}{88\%}         \\ \hline
\multicolumn{1}{c|}{\multirow{2}{*}{Binary}}            & CBOW+MLP                        & -                                            & 98.41           & 97.63           & 96.67           & 97.12           & 6.53                         & 1.46                 & \multicolumn{1}{c|}{54.87}               & \multicolumn{1}{c|}{10.44}               & \multicolumn{1}{c}{29\%}         \\
\multicolumn{1}{c|}{}                                   & MalConv                         & -                                            & 97.02           & 94.34           & 92.62           & 93.33           & \textbf{0.28}                & 227.40               & \multicolumn{1}{c|}{348.16}              & \multicolumn{1}{c|}{10.78*4}             & \multicolumn{1}{c}{37\%}         \\ \hline
\multicolumn{1}{c|}{\multirow{3}{*}{Disassembly}}       & MAGIC                           & -                                            & 98.05           & 96.75           & 94.03           & 95.14           & 13.87                        & 52.32                & \multicolumn{1}{c|}{42.02}               & \multicolumn{1}{c|}{10.61}               & \multicolumn{1}{c}{73\%}         \\
\multicolumn{1}{c|}{}                                   & Word2Vec+k-NN                   & -                                            & 98.07           & 96.41           & 96.51           & 96.45           & 109.14                       & \textbf{0.09}        & \multicolumn{1}{c|}{\textbf{6.63}}       & \multicolumn{1}{c|}{-}                   & \multicolumn{1}{c}{-}            \\
\multicolumn{1}{c|}{}                                   & MCSC                            & -                                            & 97.94           & 95.97           & 96.17           & 96.06           & 4.06                         & 3.62                 & \multicolumn{1}{c|}{45.12}               & \multicolumn{1}{c|}{10.77}               & \multicolumn{1}{c}{33\%}         \\ \hline
\bottomrule
\end{tabular}
\footnotesize
\begin{tablenotes}
 \item [1] Average Classification Performance: The prediction results of 10-fold are added up into a large confusion matrix, and Accuracy, Precision, Recall and F1-score are then calculated as a whole.
 \item[2] Resource Overhead: The resource includes virtual memory (V.Mem), GPU memory (G.Mem), and GPU-util. The V.Mem of the Word2Vec+KNN method has two values, the first one represent the resource consume for data preparation and the second one is for model training.
 \item[3] Time: The time includes data pre-processing time and model training time. The data preparation time is average time for processing a sample, and for each method is composed as follows. IMCFN: the time taken to convert a malware sample to a 224*224 size color image; CBOW+MLP: the time to delete the useless bytes from a binary file, and the time to convert the processed file to a 256*256 dimensional ascending vector matrix; MalConv: The time to process a binary file to a 2MB size; MAGIC: The time to extract an ACFG; Word2Vec+KNN: The time to parse a disassembly file into Opcode sequences, and the time to calculate the document distance between a test sample and all training samples; MCSC: The time to extract the Opcode sequence from a disassembly file and convert it to an image based on Simhash. \jj{Move to configuration part if necessary?}
\end{tablenotes}
\end{threeparttable}
\end{table*}
\end{comment}




\begin{comment}
\begin{table*}[t]
\centering
\begin{threeparttable}
\caption{Comparison of Classification Performance of Various Methods Based on 10-fold Cross-validation on BIG-15 Dataset}
\label{tab:Compare-BIG15-Non-uniform calculation criteria}
\footnotesize
\begin{tabular}{ccccccccccc}
\toprule
\hline
\multirow{2}{*}{Category}         & \multirow{2}{*}{Method} & \multicolumn{4}{c}{Average Classification Performance (\%)} & \multicolumn{3}{c}{Resource Overhead} & \multicolumn{2}{c}{Time}      \\
                                  &                         & A             & P             & R            & F1           & V.Mem (GB)    & G.Mem (GB)   & GPU    & Pre-process (s) & Train (min) \\ \hline
Image                             & IMCFN                   & 99.03         & 97.63         & 96.03        & 96.60        & 96.14         & 11.30        & 88\%   & 0.74            & 173.40      \\ \hline
\multirow{2}{*}{Binary}      & CBOW+MLP                & 98.41         & 97.73         & 96.72        & 97.05        & 54.87         & 10.95        & 29\%   & 6.53            & 1.46        \\
                                  & MalConv                 & 97.02         & 94.76         & 92.56        & 93.14        & 348.16        & 11.31 * 4    & 37\%   & 0.28            & 227.40      \\ \hline
\multirow{3}{*}{Disassembly} & MAGIC                   & 98.20         & 96.75         & 94.11        & 94.84        & 42.02         & 10.36        & 73\%   & 13.87           & 52.32       \\
                                  & Word2Vec+KNN           & 98.08         & 96.75         & 96.50        & 96.39        & 6.63   0.34   & -            & -      & 109.14 (13.91)          & 0.09        \\
                                  & MCSC                    & 97.94         & 96.02         & 96.12        & 96.04        & 45.12         & 11.30        & 33\%   & 4.06            & 3.62        \\ \hline
\bottomrule
\end{tabular}
\footnotesize
\begin{tablenotes}
 \item [1] Average Classification Performance: First, the Macro Average Scores (Precision, Recall and F1-score) of each fold are calculated, and then the 10 times results are averaged.
\end{tablenotes}
\end{threeparttable}
\end{table*}
\end{comment}




\begin{comment}
\begin{table*}[t]
\centering
\begin{threeparttable}
\caption{Comparison of Classification Performance of Various Methods Based on 10-fold Cross-validation on BIG-15 Dataset }
\label{tab:Compare-BIG15-Uniform computing standard}
\footnotesize
\begin{tabular}{ccccccccccc}
\toprule
\hline
\multirow{2}{*}{Category}    & \multirow{2}{*}{Method} & \multicolumn{4}{c}{Average Classification Performance (\%)} & \multicolumn{3}{c}{Resource Overhead} & \multicolumn{2}{c}{Time}      \\
                             &                         & A             & P             & R            & F1           & V.Mem (GB)    & G.Mem (GB)   & GPU    & Pre-process (s) & Train (min) \\ \hline
Image                        & IMCFN                   & 99.17         & 98.69         & 97.52        & 98.07        & 96.14         & 11.30        & 88\%   & 0.74            & 173.40      \\ \hline
\multirow{2}{*}{Binary}      & CBOW+MLP                & 98.41         & 97.63         & 96.67        & 97.12        & 54.87         & 10.95        & 29\%   & 6.53            & 1.46        \\
                             & MalConv                 & 97.02         & 94.34         & 92.62        & 93.33        & 348.16        & 11.31 * 4    & 37\%   & 0.28            & 227.40      \\ \hline
\multirow{3}{*}{Disassembly} & MAGIC                   & 98.05         & 96.75         & 94.03        & 95.14        & 42.02         & 10.36        & 73\%   & 13.87           & 52.32       \\
                             & Word2Vec+KNN           & 98.07         & 96.41         & 96.51        & 96.45        & 6.63   0.34   & -            & -      & 109.14 (13.91)         & 0.09        \\
                             & MCSC                    & 97.94         & 95.97         & 96.17        & 96.06        & 45.12         & 11.30        & 33\%   & 4.06            & 3.62        \\ \hline
\bottomrule
\end{tabular}
\footnotesize
\begin{tablenotes}
 \item [1] Average Classification Performance: The prediction results of 10-fold are added up into a large confusion matrix, and Accuracy, Precision, Recall and F1-score are then calculated as a whole.
 \item[2] Resource Overhead: The resource includes virtual memory (V.Mem), GPU memory (G.Mem), and GPU-util. The V.Mem of the Word2Vec+KNN method has two values, the first one represent the resource consume for data preparation and the second one is for model training.
 \item[3] Time: The time includes data pre-processing time and model training time. The data preparation time is average time for processing a sample, and for each method is composed as follows. IMCFN: the time taken to convert a malware sample to a 224*224 size color image; CBOW+MLP: the time to delete the useless bytes from a binary file, and the time to convert the processed file to a 256*256 dimensional ascending vector matrix; MalConv: The time to process a binary file to a 2MB size; MAGIC: The time to extract an ACFG; Word2Vec+KNN: The time to parse a disassembly file into Opcode sequences, and the time to calculate the document distance between a test sample and all training samples; MCSC: The time to extract the Opcode sequence from a disassembly file and convert it to an image based on Simhash. 
\end{tablenotes}
\end{threeparttable}
\end{table*}
\end{comment}

==> tab_result_Malimg.tex <==
\begin{table*}[t]
\centering
\footnotesize
\begin{threeparttable}
\caption{Performance Comparison on Malimg Dataset (10-fold cross-validation)}
\label{tab:Malimg}
\begin{tabular}{c|c|c|cccc|c|ccc}
\toprule
\hline
\multirow{2}{*}{\textbf{Category}} & \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Training Strategy}} & \multicolumn{4}{c|}{\textbf{Classification Performance (\%)}}     & \multirow{2}{*}{\textbf{Train Time (min)}} & \multicolumn{3}{c}{\textbf{Resource Overhead}} \\ \cline{4-7} \cline{9-11} 
                                   &                                 &                                             & \textbf{$A$}     & \textbf{$P_{macro}$}     & \textbf{$R_{macro}$}     & \textbf{$F1_{macro}$}    &                                            & \textbf{Mem (GB)}      & \textbf{GPU.Mem (GB)}      & \textbf{GPU (\%)}     \\ \hline
\multirow{20}{*}{Image}            & \multirow{5}{*}{ResNet-50}      & From Scratch                                & 98.14          & 95.48          & 95.06          & 95.21          & 140.02                                     & 32.77         & 10.77           & 95           \\
                                   &                                 & 10\% TL                                     & 97.34          & 93.79          & 92.77          & 93.21          & 5.29                                       & 19.46         & 10.56           & 7            \\
                                   &                                 & 50\% TL                                     & 98.02          & 95.61          & 94.46          & 94.93          & 29.61                                      & 19.46         & 10.56           & 5            \\
                                   &                                 & 80\% TL                                     & \textbf{98.59} & \textbf{96.37} & \textbf{96.23} & \textbf{96.29} & 44.65                                      & 19.46         & 10.56           & 8            \\
                                   &                                 & 100\% TL                                    & 98.49          & 96.33          & 95.88          & 96.10          & 70.80                                      & 20.48         & 10.56           & 7            \\ \cline{2-11} 
                                   & \multirow{5}{*}{VGG-16}         & From Scratch                                & \textbf{99.08} & \textbf{97.71} & \textbf{97.74} & \textbf{97.73} & 58.63                                      & 32.77         & 10.77           & 94           \\
                                   &                                 & 10\% TL                                     & 96.37          & 90.05          & 89.24          & 89.50          & 2.40                                       & 17.41         & 10.44           & 7            \\
                                   &                                 & 50\% TL                                     & 97.24          & 91.29          & 91.64          & 91.41          & 7.32                                       & 16.38         & 10.44           & 5            \\
                                   &                                 & 80\% TL                                     & 98.58          & 96.35          & 96.23          & 96.28          & 11.46                                      & 17.41         & 10.44           & 20           \\
                                   &                                 & 100\% TL                                    & 98.63          & 96.47          & 96.40          & 96.42          & 14.16                                      & 19.46         & 10.44           & 52           \\ \cline{2-11} 
                                   & \multirow{5}{*}{Inception-V3}   & From Scratch                                & \textbf{97.77} & \textbf{96.29} & \textbf{93.82} & \textbf{93.98} & 273.12                                     & 32.77         & 10.77           & 94           \\
                                   &                                 & 10\% TL                                     & 93.82          & 87.07          & 83.93          & 85.05          & 3.93                                       & 16.38         & 10.56           & 6            \\
                                   &                                 & 50\% TL                                     & 95.75          & 89.23          & 88.63          & 88.86          & 11.04                                      & 17.41         & 10.56           & 2            \\
                                   &                                 & 80\% TL                                     & 96.17          & 90.15          & 89.61          & 89.84          & 16.32                                      & 20.48         & 10.56           & 12           \\
                                   &                                 & 100\% TL                                    & 96.43          & 90.62          & 90.28          & 90.41          & 18.96                                      & 18.43         & 10.56           & 7            \\ \cline{2-11} 
                                   & \multirow{5}{*}{IMCFN}          & From Scratch                                & \textbf{99.13} & \textbf{98.08} & \textbf{97.62} & \textbf{97.84} & 34.95                                      & 43.01         & 10.77           & 96           \\
                                   &                                 & 10\% TL                                     & 91.48          & 74.18          & 74.05          & 73.35          & 4.63                                       & 18.43         & 10.44           & 26           \\
                                   &                                 & 50\% TL                                     & 96.67          & 90.70          & 90.06          & 90.27          & 12.66                                      & 22.52         & 10.44           & 35           \\
                                   &                                 & 80\% TL                                     & 96.96          & 91.17          & 90.85          & 90.93          & 18.41                                      & 22.53         & 10.44           & 39           \\
                                   &                                 & 100\% TL                                    & 97.13          & 91.29          & 91.33          & 91.25          & 18.55                                      & 23.55         & 10.44           & 40           \\ \hline \bottomrule
\end{tabular}
\footnotesize
\end{threeparttable}
\end{table*}











\begin{comment}
\begin{table*}[t]
\centering
\footnotesize
\begin{threeparttable}
\caption{Comparison of Classification Performance of Various Methods Based on 10-fold Cross-validation on the Malimg Dataset}
\label{tab:Malimg-11}
\begin{tabular}{c|c|c|cccc|c|ccc}
\toprule
\hline
                                    &                                  &                                              & \multicolumn{4}{c|}{\textbf{Classification Performance (\%)}}                                                             &                                             & \multicolumn{3}{c}{\textbf{Resource Overhead}}                                          \\ \cline{4-7} \cline{9-11} 
\multirow{-2}{*}{\textbf{Category}} & \multirow{-2}{*}{\textbf{Model}} & \multirow{-2}{*}{\textbf{Training Strategy}} & \textbf{A}                   & \textbf{P}                   & \textbf{R}                   & \textbf{F1}                  & \multirow{-2}{*}{\textbf{Train Time (min)}} & Mem (GB)                     & G.Mem (GB)                   & GPU (\%)                  \\ \hline
                                    &                                  & From Scratch                                 & 98.14                        & 95.48                        & 95.06                        & 95.21                        & 140.02                                      & 32.77                        & 10.77                        & 95                        \\
                                    &                                  & 10\% TL                                      & 97.34                        & 93.79                        & 92.77                        & 93.21                        & 5.29                                        & 19.46                        & 10.56                        & 7                         \\
                                    &                                  & 50\% TL                                      & 98.02                        & 95.61                        & 94.46                        & 94.93                        & 29.61                                       & 19.46                        & 10.56                        & 5                         \\
                                    &                                  & 80\% TL                                      & \textbf{98.59}               & \textbf{96.37}               & \textbf{96.23}               & \textbf{96.29}               & 44.65                                       & 19.46                        & 10.56                        & 8                         \\
                                    & \multirow{-5}{*}{ResNet-50}      & 100\% TL                                     & 98.49                        & 96.33                        & 95.88                        & 96.10                        & 70.80                                       & 20.48                        & 10.56                        & 7                         \\ \cline{2-11} 
                                    &                                  & From Scratch                                 & \textbf{99.08}               & \textbf{97.71}               & \textbf{97.74}               & \textbf{97.73}               & 58.63                                       & 32.77                        & 10.77                        & 94                        \\
                                    &                                  & 10\% TL                                      & 96.37                        & 90.05                        & 89.24                        & 89.50                        & 2.40                                        & 17.41                        & 10.44                        & 7                         \\
                                    &                                  & 50\% TL                                      & 97.24                        & 91.29                        & 91.64                        & 91.41                        & 7.32                                        & 16.38                        & 10.44                        & 5                         \\
                                    &                                  & 80\% TL                                      & 98.58                        & 96.35                        & 96.23                        & 96.28                        & 11.46                                       & 17.41                        & 10.44                        & 20                        \\
                                    & \multirow{-5}{*}{VGG-16}         & 100\% TL                                     & 98.63                        & 96.47                        & 96.40                        & 96.42                        & 14.16                                       & 19.46                        & 10.44                        & 52                        \\ \cline{2-11} 
                                    &                                  & From Scratch                                 & \textbf{97.77}               & \textbf{96.29}               & \textbf{93.82}               & \textbf{93.98}               & 273.12                                      & 32.77                        & 10.77                        & 94                        \\
                                    &                                  & 10\% TL                                      & 93.82                        & 87.07                        & 83.93                        & 85.05                        & 3.93                                        & 16.38                        & 10.56                        & 6                         \\
                                    &                                  & 50\% TL                                      & 95.75                        & 89.23                        & 88.63                        & 88.86                        & 11.04                                       & 17.41                        & 10.56                        & 2                         \\
                                    &                                  & 80\% TL                                      & 96.17                        & 90.15                        & 89.61                        & 89.84                        & 16.32                                       & 20.48                        & 10.56                        & 12                        \\
                                    & \multirow{-5}{*}{Inception-V3}   & 100\% TL                                     & 96.43                        & 90.62                        & 90.28                        & 90.41                        & 18.96                                       & 18.43                        & 10.56                        & 7                         \\ \cline{2-11} 
                                    &                                  & From Scratch                                 & \textbf{99.13}               & \textbf{98.08}               & \textbf{97.62}               & \textbf{97.84}               & 34.95                                       & 43.01                        & 10.77                        & 96                        \\ \cline{3-11} 
                                    &                                  & {\color[HTML]{FE0000} 10\% TL}               & {\color[HTML]{FE0000} 91.48} & {\color[HTML]{FE0000} 74.18} & {\color[HTML]{FE0000} 74.05} & {\color[HTML]{FE0000} 73.35} & {\color[HTML]{FE0000} 4.63}                 & {\color[HTML]{FE0000} 18.43} & {\color[HTML]{FE0000} 10.44} & {\color[HTML]{FE0000} 26} \\
                                    &                                  & {\color[HTML]{FE0000} 50\% TL}               & {\color[HTML]{FE0000} 96.67} & {\color[HTML]{FE0000} 90.70} & {\color[HTML]{FE0000} 90.06} & {\color[HTML]{FE0000} 90.27} & {\color[HTML]{FE0000} 12.66}                & {\color[HTML]{FE0000} 22.52} & {\color[HTML]{FE0000} 10.44} & {\color[HTML]{FE0000} 35} \\
                                    &                                  & {\color[HTML]{FE0000} 80\% TL}               & {\color[HTML]{FE0000} 96.96} & {\color[HTML]{FE0000} 91.17} & {\color[HTML]{FE0000} 90.85} & {\color[HTML]{FE0000} 90.93} & {\color[HTML]{FE0000} 18.41}                & {\color[HTML]{FE0000} 22.53} & {\color[HTML]{FE0000} 10.44} & {\color[HTML]{FE0000} 39} \\
                                    &                                  & {\color[HTML]{FE0000} 100\% TL}              & {\color[HTML]{FE0000} 97.13} & {\color[HTML]{FE0000} 91.29} & {\color[HTML]{FE0000} 91.33} & {\color[HTML]{FE0000} 91.25} & {\color[HTML]{FE0000} 18.55}                & {\color[HTML]{FE0000} 23.55} & {\color[HTML]{FE0000} 10.44} & {\color[HTML]{FE0000} 40} \\ \cline{3-11} 
                                    &                                  & 10\% TL                                      & 97.19                        & 94.41                        & 91.82                        & 92.60                        & 12.64                                       & 39.94                        & 10.77                        & 88                        \\
                                    &                                  & 50\% TL                                      & 98.64                        & 96.41                        & \multicolumn{1}{l}{96.35}    & 96.37                        & 16.60                                       & 48.13                        & 10.77                        & 90                        \\
                                    &                                  & 80\% TL                                      & 99.00                        & 97.42                        & 97.40                        & 97.41                        & 22.59                                       & 49.15                        & 10.77                        & 92                        \\
\multirow{-24}{*}{Image}            & \multirow{-9}{*}{IMCFN}          & 100\% TL                                     & 99.08                        & 97.62                        & 97.57                        & 97.59                        & 21.75                                       & 50.18                        & 10.77                        & 91                        \\ \hline
\bottomrule
\end{tabular}
\footnotesize
\yx{red data: IMCFN doesn't open the last feature extraction block (setting is consistent with other models). 
~\\
black data: IMCFN open the last feature extraction block.
~\\
Malimg dataset is imbalanced.}
\end{threeparttable}
\end{table*}
\end{comment}









\begin{comment}
\begin{table*}[t]
\centering
\footnotesize
\begin{threeparttable}
\caption{Comparison of Classification Performance of Various Methods Based on 10-fold Cross-validation on the Malimg Dataset}
\label{tab:Malimg-2}
\begin{tabular}{c|c|c|cccc|c|ccc}
\toprule
\hline
\multirow{2}{*}{\textbf{Category}} & \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Training Strategy}} & \multicolumn{4}{c|}{\textbf{Classification Performance (\%)}}                & \multirow{2}{*}{\textbf{Train Time (min)}} & \multicolumn{3}{c}{\textbf{Resource Overhead}} \\ \cline{4-7} \cline{9-11} 
                                   &                                 &                                             & \textbf{A}     & \textbf{P}     & \textbf{R}                & \textbf{F1}    &                                            & Mem (GB)      & G.Mem (MiB)     & GPU (\%)     \\ \hline
\multirow{20}{*}{Image}            & \multirow{5}{*}{ResNet-50}      & From Scratch                                & 98.14          & 95.48          & 95.06                     & 95.21          & 140.02                                     & 32.77         & 10.77           & 95           \\
                                   &                                 & 10\% TL                                     & 97.34          & 93.79          & 92.77                     & 93.21          & 5.29                                       & 19.46         & 10.56           & 7            \\
                                   &                                 & 50\% TL                                     & 98.02          & 95.61          & 94.46                     & 94.93          & 29.61                                      & 19.46         & 10.56           & 5            \\
                                   &                                 & 80\% TL                                     & \textbf{98.59} & \textbf{96.37} & \textbf{96.23}            & \textbf{96.29} & 44.65                                      & 19.46         & 10.56           & 8            \\
                                   &                                 & 100\% TL                                    & 98.49          & 96.33          & 95.88                     & 96.10          & 70.80                                      & 20.48         & 10.56           & 7            \\ \cline{2-11} 
                                   & \multirow{5}{*}{VGG-16}         & From Scratch                                & \textbf{99.08} & \textbf{97.71} & \textbf{97.74}            & \textbf{97.73} & 58.63                                      & 32.77         & 10.77           & 94           \\
                                   &                                 & 10\% TL                                     & 96.37          & 90.05          & 89.24                     & 89.50          & 2.40                                       & 17.41         & 10.44           & 7            \\
                                   &                                 & 50\% TL                                     & 97.24          & 91.29          & 91.64                     & 91.41          & 7.32                                       & 16.38         & 10.44           & 5            \\
                                   &                                 & 80\% TL                                     & 98.58          & 96.35          & 96.23                     & 96.28          & 11.46                                      & 17.41         & 10.44           & 20           \\
                                   &                                 & 100\% TL                                    & 98.63          & 96.47          & 96.40                     & 96.42          & 14.16                                      & 19.46         & 10.44           & 52           \\ \cline{2-11} 
                                   & \multirow{5}{*}{Inception-V3}   & From Scratch                                & \textbf{97.77} & \textbf{96.29} & \textbf{93.82}            & \textbf{93.98} & 273.12                                     & 32.77         & 10.77           & 94           \\
                                   &                                 & 10\% TL                                     & 93.82          & 87.07          & 83.93                     & 85.05          & 3.93                                       & 16.38         & 10.56           & 6            \\
                                   &                                 & 50\% TL                                     & 95.75          & 89.23          & 88.63                     & 88.86          & 11.04                                      & 17.41         & 10.56           & 2            \\
                                   &                                 & 80\% TL                                     & 96.17          & 90.15          & 89.61                     & 89.84          & 16.32                                      & 20.48         & 10.56           & 12           \\
                                   &                                 & 100\% TL                                    & 96.43          & 90.62          & 90.28                     & 90.41          & 18.96                                      & 18.43         & 10.56           & 7            \\ \cline{2-11} 
                                   & \multirow{5}{*}{IMCFN}          & From Scratch                                & \textbf{99.13} & \textbf{98.08} & \textbf{97.62}            & \textbf{97.84} & 34.95                                      & 43.01         & 10.77           & 96           \\
                                   &                                 & 10\% TL                                     & 97.19          & 94.41          & 91.82                     & 92.60          & 12.64                                      & 39.94         & 10.77           & 88           \\
                                   &                                 & 50\% TL                                     & 98.64          & 96.41          & \multicolumn{1}{l}{96.35} & 96.37          & 16.60                                      & 48.13         & 10.77           & 90           \\
                                   &                                 & 80\% TL                                     & 99.00          & 97.42          & 97.40                     & 97.41          & 22.59                                      & 49.15         & 10.77           & 92           \\
                                   &                                 & 100\% TL                                    & 99.08          & 97.62          & 97.57                     & 97.59(\yx{91.51$^\star$})           & 21.75                                      & 50.18         & 10.77           & 91           \\ \hline
\bottomrule
\end{tabular}
\footnotesize
\yx{$^\star$ IMCFN doesn't open the last feature extraction block (setting is consistent with other models). IMCFN is not the best in 100\% TL compared with other models.
~\\
Malimg dataset is imbalanced.}
\end{threeparttable}
\end{table*}
\end{comment}

















\begin{comment}
\begin{table*}[t]
\centering\scriptsize
\begin{threeparttable}
\caption{Comparison of Classification Performance of Various Methods Based on 10-fold Cross-validation on the Malimg Dataset}
\label{tab:Compare-Malimg-early stop epoch}
\begin{tabular}{c|c|c|cccc|c}
\toprule
\hline
\multirow{2}{*}{\textbf{Category}} & \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Training Strategy}} & \multicolumn{4}{c|}{\textbf{Classification Performance (\%)}}                & \textbf{Time}        \\ \cline{4-8} 
                                   &                                 &                                             & \textbf{A}     & \textbf{P}     & \textbf{R}                & \textbf{F1}    & \textbf{Train (min)} \\ \hline
\multirow{20}{*}{Image}            & \multirow{5}{*}{ResNet-50}      & From Scratch                                & 98.14          & 95.48          & 95.06                     & 95.21          & 140.02               \\
                                   &                                 & 10\%-Transfer                               & 97.34          & 93.79          & 92.77                     & 93.21          & 5.29                 \\
                                   &                                 & 50\%-Transfer                               & 98.02          & 95.61          & 94.46                     & 94.93          & 29.61                \\
                                   &                                 & 80\%-Transfer                               & \textbf{98.59} & \textbf{96.37} & \textbf{96.23}            & \textbf{96.29} & 44.65                \\
                                   &                                 & 100\%-Transfer                              & 98.49          & 96.33          & 95.88                     & 96.10          & 70.80                \\ \cline{2-8} 
                                   & \multirow{5}{*}{VGG-16}         & From Scratch                                & \textbf{99.08} & \textbf{97.71} & \textbf{97.74}            & \textbf{97.73} & 58.63                \\
                                   &                                 & 10\%-Transfer                               & 96.37          & 90.05          & 89.24                     & 89.50          & 2.40                 \\
                                   &                                 & 50\%-Transfer                               & 97.24          & 91.29          & 91.64                     & 91.41          & 7.32                 \\
                                   &                                 & 80\%-Transfer                               & 98.58          & 96.35          & 96.23                     & 96.28          & 11.46                \\
                                   &                                 & 100\%-Transfer                              & 98.63          & 96.47          & 96.40                     & 96.42          & 14.16                \\ \cline{2-8} 
                                   & \multirow{5}{*}{Inception-V3}   & From Scratch                                & \textbf{97.77} & \textbf{96.29} & \textbf{93.82}            & \textbf{93.98} & 273.12               \\
                                   &                                 & 10\%-Transfer                               & 93.82          & 87.07          & 83.93                     & 85.05          & 3.93                 \\
                                   &                                 & 50\%-Transfer                               & 95.75          & 89.23          & 88.63                     & 88.86          & 11.04                \\
                                   &                                 & 80\%-Transfer                               & 96.17          & 90.15          & 89.61                     & 89.84          & 16.32                \\
                                   &                                 & 100\%-Transfer                              & 96.43          & 90.62          & 90.28                     & 90.41          & 18.96                \\ \cline{2-8} 
                                   & \multirow{5}{*}{IMCFN}          & From Scratch                                & \textbf{99.13} & \textbf{98.08} & \textbf{97.62}            & \textbf{97.84} & 34.95                \\
                                   &                                 & 10\%-Transfer                               & 97.19          & 94.41          & 91.82                     & 92.60          & 12.64                \\
                                   &                                 & 50\%-Transfer                               & 98.64          & 96.41          & \multicolumn{1}{l}{96.35} & 96.37          & 16.60                \\
                                   &                                 & 80\%-Transfer                               & 99.00          & 97.42          & 97.40                     & 97.41          & 22.59                \\
                                   &                                 & 100\%-Transfer                              & 99.08          & 97.62          & 97.57                     & 97.59        & 21.75                \\ \hline
\bottomrule
\end{tabular}
\footnotesize
\end{threeparttable}
\end{table*}
\end{comment}



























\begin{comment}
\begin{table*}[t]
\centering\scriptsize
\begin{threeparttable}
\caption{Comparison of Classification Performance of Various Methods Based on 10-fold Cross-validation on the Malimg Dataset}
\label{tab:Compare-Malimg-the original epoch}
\begin{tabular}{l|c|c|cccc|c|c|}
\toprule
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Category}}} & \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Training Strategy}}  & \multicolumn{4}{c|}{\textbf{Classification Performance (\%)}}     & \multicolumn{2}{c|}{\textbf{Time}}     \\ \cline{4-9} 
\multicolumn{1}{c|}{}                                   &                                 &                                              & \textbf{A}     & \textbf{P}     & \textbf{R}     & \textbf{F1}    & \textbf{Pre(s)} & \textbf{Train (min)} \\ \hline
\multirow{20}{*}{Image}                                 & \multirow{5}{*}{ResNet-50}      & Train From Scretch                           & 98.14          & 95.48          & 95.06          & 95.21          &                 & 175.02               \\
                                                        &                                 & 10\%-Transfer Learning                       & 97.34          & 93.79          & 92.77          & 93.21          &                 & 15.12                \\
                                                        &                                 & 50\%-Transfer Learning                       & 98.02          & 95.61          & 94.46          & 94.93          & \textbf{}       & 42.30                \\
                                                        &                                 & 80\%-Transfer Learning                       & 98.59          & 96.37          & 96.23          & 96.29          &                 & 63.78                \\
                                                        &                                 & \multicolumn{1}{l|}{100\%-Transfer Learning} & 98.49          & 96.33          & 95.88          & 96.10          &                 & 70.80                \\ \cline{2-7} \cline{9-9} 
                                                        & \multirow{5}{*}{VGG-16}         & Train From Scretch                           & 99.08          & 97.71          & \textbf{97.74} & 97.73          &                 & 94.56                \\
                                                        &                                 & 10\%-Transfer Learning                       & 96.37          & 90.05          & 89.24          & 89.50          & \textbf{}       & 2.40                 \\
                                                        &                                 & 50\%-Transfer Learning                       & 97.24          & 91.29          & 91.64          & 91.41          & \textbf{}       & 7.32                 \\
                                                        &                                 & 80\%-Transfer Learning                       & 98.58          & 96.35          & 96.23          & 96.28          & \textbf{}       & 11.46                \\
                                                        &                                 & \multicolumn{1}{l|}{100\%-Transfer Learning} & 98.63          & 96.47          & 96.40          & 96.42          & \textbf{}       & 14.16                \\ \cline{2-7}
                                                        & \multirow{5}{*}{Inception-V3}   & Train From Scretch                           & 97.77          & 96.29          & 93.82          & 93.98          & \textbf{}       & 273.12               \\
                                                        &                                 & 10\%-Transfer Learning                       & 93.82          & 87.07          & 83.93          & 85.05          &                 & 3.93                 \\
                                                        &                                 & 50\%-Transfer Learning                       & 95.75          & 89.23          & 88.63          & 88.86          & \textbf{}       & 11.04                \\
                                                        &                                 & 80\%-Transfer Learning                       & 96.17          & 90.15          & 89.61          & 89.84          &                 & 16.32                \\
                                                        &                                 & \multicolumn{1}{l|}{100\%-Transfer Learning} & 96.43          & 90.62          & 90.28          & 90.41          & \textbf{}       & 18.96                \\ \cline{2-7}
                                                        & \multirow{5}{*}{IMCFN}          & Train From Scretch                           & \textbf{99.13} & \textbf{98.08} & 97.62          & \textbf{97.84} & \textbf{}       & 79.44                \\
                                                        &                                 & 10\%-Transfer Learning                       & 97.19          & 94.41          & 91.82          & 92.60          &                 & 26.34                \\
                                                        &                                 & 50\%-Transfer Learning                       & 98.64          & 96.41          & 96.35          & 96.37          &                 & 79.80                \\
                                                        &                                 & 80\%-Transfer Learning                       & 99.00          & 97.42          & 97.40          & 97.41          & \textbf{}       & 117.66               \\
                                                        &                                 & \multicolumn{1}{l|}{100\%-Transfer Learning} & 99.08          & 97.62          & 97.57          & 97.59          &                 & 146.94               \\ \hline
\bottomrule
\end{tabular}
\footnotesize
\end{threeparttable}
\end{table*}
\end{comment}

==> tab_result_MalwareBazaar.tex <==
\begin{table*}[t]
\centering\footnotesize
\begin{threeparttable}
\caption{Performance Comparison on MalwareBazaar Dataset (10-fold cross-validation)}
\label{tab:MalwareBazaar}
\begin{tabular}{c|c|c|cccc|c|ccc}
\toprule
\hline
\multirow{2}{*}{\textbf{Category}} & \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Training Strategy}} & \multicolumn{4}{c|}{\textbf{Classification Performance (\%)}}     & \multirow{2}{*}{\textbf{Train Time (min)}} & \multicolumn{3}{c}{\textbf{Reasource Overhead}}                                                       \\ \cline{4-7} \cline{9-11} 
                                   &                                 &                                             & \textbf{$A$}     & \textbf{$P_{macro}$}     & \textbf{$R_{macro}$}     & \textbf{$F1_{macro}$}    &                                            & \multicolumn{1}{c|}{\textbf{Mem (GB)}} & \multicolumn{1}{c|}{\textbf{GPU.Mem (GB)}} & \textbf{GPU (\%)} \\ \hline
\multirow{20}{*}{Image}            & \multirow{5}{*}{ResNet-50}      & From Scratch                                & \textbf{96.68} & \textbf{96.91} & \textbf{96.75} & \textbf{96.83} & 8.35                                       & \multicolumn{1}{c|}{17.41}             & \multicolumn{1}{c|}{10.77}               & 95                \\
                                   &                                 & 10\% TL                                     & 90.03          & 89.48          & 90.99          & 90.09          & 4.07                                       & \multicolumn{1}{c|}{9.14}              & \multicolumn{1}{c|}{10.56}               & 6                 \\
                                   &                                 & 50\% TL                                     & 93.98          & 94.28          & 94.57          & 94.38          & 7.23                                       & \multicolumn{1}{c|}{9.13}              & \multicolumn{1}{c|}{10.56}               & 7                 \\
                                   &                                 & 80\% TL                                     & 94.90          & 95.21          & 95.34          & 95.25          & 9.11                                       & \multicolumn{1}{c|}{9.16}              & \multicolumn{1}{c|}{10.56}               & 5                 \\
                                   &                                 & 100\% TL                                    & 95.30          & 95.66          & 95.68          & 95.65          & 10.01                                      & \multicolumn{1}{c|}{9.19}              & \multicolumn{1}{c|}{10.56}               & 6                 \\ \cline{2-11} 
                                   & \multirow{5}{*}{VGG-16}         & From Scratch                                & \textbf{96.35} & \textbf{96.58} & \textbf{96.54} & \textbf{96.56} & 43.96                                      & \multicolumn{1}{c|}{18.43}             & \multicolumn{1}{c|}{10.77}               & 97                \\
                                   &                                 & 10\% TL                                     & 83.55          & 86.50          & 76.12          & 76.80          & 1.16                                       & \multicolumn{1}{c|}{8.17}              & \multicolumn{1}{c|}{10.44}               & 56                \\
                                   &                                 & 50\% TL                                     & 92.35          & 92.75          & 92.54          & 92.51          & 2.19                                       & \multicolumn{1}{c|}{9.34}              & \multicolumn{1}{c|}{10.44}               & 52                \\
                                   &                                 & 80\% TL                                     & 93.85          & 93.92          & 94.37          & 94.06          & 2.98                                       & \multicolumn{1}{c|}{10.24}             & \multicolumn{1}{c|}{10.44}               & 55                \\
                                   &                                 & 100\% TL                                    & 94.43          & 94.43          & 94.90          & 94.60          & 3.94                                       & \multicolumn{1}{c|}{11.26}             & \multicolumn{1}{c|}{10.44}               & 52                \\ \cline{2-11} 
                                   & \multirow{5}{*}{Inception-V3}   & From Scratch                                & \textbf{95.83} & \textbf{95.67} & \textbf{95.79} & \textbf{95.73} & 6.39                                       & \multicolumn{1}{c|}{12.29}             & \multicolumn{1}{c|}{10.77}               & 96                \\
                                   &                                 & 10\% TL                                     & 90.28          & 90.87          & 90.99          & 90.87          & 0.79                                       & \multicolumn{1}{c|}{7.83}              & \multicolumn{1}{c|}{10.56}               & 7                 \\
                                   &                                 & 50\% TL                                     & 93.75          & 94.31          & 94.20          & 94.24          & 3.77                                       & \multicolumn{1}{c|}{8.13}              & \multicolumn{1}{c|}{10.56}               & 8                 \\
                                   &                                 & 80\% TL                                     & 94.48          & 94.96          & 94.87          & 94.90          & 6.37                                       & \multicolumn{1}{c|}{8.70}              & \multicolumn{1}{c|}{10.56}               & 6                 \\
                                   &                                 & 100\% TL                                    & 94.80          & 95.15          & 95.17          & 95.15          & 8.47                                       & \multicolumn{1}{c|}{8.47}              & \multicolumn{1}{c|}{10.56}               & 7                 \\ \cline{2-11} 
                                   & \multirow{5}{*}{IMCFN}          & From Scratch                                & \textbf{97.38} & \textbf{97.53} & \textbf{97.41} & \textbf{97.47} & 18.75                                      & \multicolumn{1}{c|}{22.53}             & \multicolumn{1}{c|}{10.77}               & 92                \\
                                   &                                 & 10\% TL                                     & 91.30          & 91.72          & 91.27          & 91.35          & 2.14                                       & \multicolumn{1}{c|}{9.39}              & \multicolumn{1}{c|}{10.44}               & 27                \\
                                   &                                 & 50\% TL                                     & 94.95          & 94.99          & 95.33          & 95.10          & 5.75                                       & \multicolumn{1}{c|}{10.24}             & \multicolumn{1}{c|}{10.44}               & 37                \\
                                   &                                 & 80\% TL                                     & 95.55          & 95.59          & 95.86          & 95.68          & 6.25                                       & \multicolumn{1}{c|}{11.26}             & \multicolumn{1}{c|}{10.44}               & 45                \\
                                   &                                 & 100\% TL                                    & 95.73          & 95.73          & 96.02          & 95.84          & 7.76                                       & \multicolumn{1}{c|}{11.26}             & \multicolumn{1}{c|}{10.44}               & 37                \\ \hline
\multirow{2}{*}{Binary}            & CBOW+MLP                        & -                                           & \textbf{97.81} & \textbf{97.92} & \textbf{98.08} & \textbf{98.00} & 0.82                                       & \multicolumn{1}{c|}{51.94}             & \multicolumn{1}{c|}{10.44}               & 34                \\
                                   & MalConv                         & -                                           & 95.92          & 96.04          & 96.43          & 96.20          & 65.40                                      & \multicolumn{1}{c|}{246.78}            & \multicolumn{1}{c|}{10.78}               & 60                \\ \hline
\multirow{3}{*}{Disassembly}       & MAGIC                           & -                                           & 92.82          & 88.03          & 87.36          & 87.45          & 246.00                                     & \multicolumn{1}{c|}{113.66}            & \multicolumn{1}{c|}{10.61}               & 81                \\
                                   & Word2Vec+KNN                    & -                                           & 95.64          & 93.34          & 94.29          & 93.79          &  \approx0                                          & \multicolumn{1}{c|}{5.54}              & \multicolumn{1}{c|}{-}                   & -                 \\
                                   & MCSC                            & -                                           & \textbf{96.80} & \textbf{94.97} & \textbf{94.51} & \textbf{94.70} & 1.07                                       & \multicolumn{1}{c|}{45.34}             & \multicolumn{1}{c|}{10.77}               & 33                \\ \hline \bottomrule
\end{tabular}
\footnotesize
\end{threeparttable}
\end{table*}





































\begin{comment}
\begin{table*}[t]
\centering\footnotesize
\begin{threeparttable}
\caption{Comparison of Classification Performance of Various Methods Based on 10-fold Cross-validation on the MalwareBazaar Dataset\jj{Transfer Learning can be shortened, such as TL to save space and for clarity.} \yx{Done.}}
\label{tab:MalwareBazaar-11}
\begin{tabular}{c|c|c|cccc|c|ccc}
\toprule
\hline
                                    &                                                                                 &                                              & \multicolumn{4}{c|}{\textbf{Classification Performance (\%)}}                                                             &                                             & \multicolumn{3}{c}{\textbf{Reasource Overhead}}                                                                                   \\ \cline{4-7} \cline{9-11} 
\multirow{-2}{*}{\textbf{Category}} & \multirow{-2}{*}{\textbf{Model}}                                                & \multirow{-2}{*}{\textbf{Training Strategy}} & \textbf{A}                   & \textbf{P}                   & \textbf{R}                   & \textbf{F1}                  & \multirow{-2}{*}{\textbf{Train Time (min)}} & \multicolumn{1}{c|}{\textbf{Mem (GB)}}            & \multicolumn{1}{c|}{\textbf{G.Mem (GB)}}          & \textbf{GPU (\%)}         \\ \hline
                                    &                                                                                 & From Scratch                                 & \textbf{96.68}               & \textbf{96.91}               & \textbf{96.75}               & \textbf{96.83}               & 8.35                                        & \multicolumn{1}{c|}{17.41}                        & \multicolumn{1}{c|}{10.77}                        & 95                        \\
                                    &                                                                                 & 10\% TL                                      & 90.03                        & 89.48                        & 90.99                        & 90.09                        & 4.07                                        & \multicolumn{1}{c|}{9.14}                         & \multicolumn{1}{c|}{10.56}                        & 6                         \\
                                    &                                                                                 & 50\% TL                                      & 93.98                        & 94.28                        & 94.57                        & 94.38                        & 7.23                                        & \multicolumn{1}{c|}{9.13}                         & \multicolumn{1}{c|}{10.56}                        & 7                         \\
                                    &                                                                                 & 80\% TL                                      & 94.90                        & 95.21                        & 95.34                        & 95.25                        & 9.11                                        & \multicolumn{1}{c|}{9.16}                         & \multicolumn{1}{c|}{10.56}                        & 5                         \\
                                    & \multirow{-5}{*}{ResNet-50}                                                     & 100\% TL                                     & 95.30                        & 95.66                        & 95.68                        & 95.65                        & 10.01                                       & \multicolumn{1}{c|}{9.19}                         & \multicolumn{1}{c|}{10.56}                        & 6                         \\ \cline{2-11} 
                                    &                                                                                 & From Scratch                                 & \textbf{96.35}               & \textbf{96.58}               & \textbf{96.54}               & \textbf{96.56}               & 43.96                                       & \multicolumn{1}{c|}{18.43}                        & \multicolumn{1}{c|}{10.77}                        & 97                        \\
                                    &                                                                                 & 10\% TL                                      & 83.55                        & 86.50                        & 76.12                        & 76.80                        & 1.16                                        & \multicolumn{1}{c|}{8.17}                         & \multicolumn{1}{c|}{10.44}                        & 56                        \\
                                    &                                                                                 & 50\% TL                                      & 92.35                        & 92.75                        & 92.54                        & 92.51                        & 2.19                                        & \multicolumn{1}{c|}{9.34}                         & \multicolumn{1}{c|}{10.44}                        & 52                        \\
                                    &                                                                                 & 80\% TL                                      & 93.85                        & 93.92                        & 94.37                        & 94.06                        & 2.98                                        & \multicolumn{1}{c|}{10.24}                        & \multicolumn{1}{c|}{10.44}                        & 55                        \\
                                    & \multirow{-5}{*}{VGG-16}                                                        & 100\% TL                                     & 94.43                        & 94.43                        & 94.90                        & 94.60                        & 3.94                                        & \multicolumn{1}{c|}{11.26}                        & \multicolumn{1}{c|}{10.44}                        & 52                        \\ \cline{2-11} 
                                    &                                                                                 & From Scratch                                 & \textbf{95.83}               & \textbf{95.67}               & \textbf{95.79}               & \textbf{95.73}               & 6.39                                        & \multicolumn{1}{c|}{12.29}                        & \multicolumn{1}{c|}{10.77}                        & 96                        \\
                                    &                                                                                 & 10\% TL                                      & 90.28                        & 90.87                        & 90.99                        & 90.87                        & 0.79                                        & \multicolumn{1}{c|}{7.83}                         & \multicolumn{1}{c|}{10.56}                        & 7                         \\
                                    &                                                                                 & 50\% TL                                      & 93.75                        & 94.31                        & 94.20                        & 94.24                        & 3.77                                        & \multicolumn{1}{c|}{8.13}                         & \multicolumn{1}{c|}{10.56}                        & 8                         \\
                                    &                                                                                 & 80\% TL                                      & 94.48                        & 94.96                        & 94.87                        & 94.90                        & 6.37                                        & \multicolumn{1}{c|}{8.70}                         & \multicolumn{1}{c|}{10.56}                        & 6                         \\
                                    & \multirow{-5}{*}{Inception-V3}                                                  & 100\% TL                                     & 94.80                        & 95.15                        & 95.17                        & 95.15                        & 8.47                                        & \multicolumn{1}{c|}{8.47}                         & \multicolumn{1}{c|}{10.56}                        & 7                         \\ \cline{2-11} 
                                    &                                                                                 & From Scratch                                 & \textbf{97.38}               & \textbf{97.53}               & \textbf{97.41}               & \textbf{97.47}               & 18.75                                       & \multicolumn{1}{c|}{22.53}                        & \multicolumn{1}{c|}{10.77}                        & 92                        \\ \cline{3-11} 
                                    &                                                                                 & {\color[HTML]{FE0000} 10\% TL}               & {\color[HTML]{FE0000} 91.30} & {\color[HTML]{FE0000} 91.72} & {\color[HTML]{FE0000} 91.27} & {\color[HTML]{FE0000} 91.35} & {\color[HTML]{FE0000} 2.14}                 & \multicolumn{1}{c|}{{\color[HTML]{FE0000} 9.39}}  & \multicolumn{1}{c|}{{\color[HTML]{FE0000} 10.44}} & {\color[HTML]{FE0000} 27} \\
                                    &                                                                                 & {\color[HTML]{FE0000} 50\% TL}               & {\color[HTML]{FE0000} 94.95} & {\color[HTML]{FE0000} 94.99} & {\color[HTML]{FE0000} 95.33} & {\color[HTML]{FE0000} 95.10} & {\color[HTML]{FE0000} 5.75}                 & \multicolumn{1}{c|}{{\color[HTML]{FE0000} 10.24}} & \multicolumn{1}{c|}{{\color[HTML]{FE0000} 10.44}} & {\color[HTML]{FE0000} 37} \\
                                    &                                                                                 & {\color[HTML]{FE0000} 80\% TL}               & {\color[HTML]{FE0000} 95.55} & {\color[HTML]{FE0000} 95.59} & {\color[HTML]{FE0000} 95.86} & {\color[HTML]{FE0000} 95.68} & {\color[HTML]{FE0000} 6.25}                 & \multicolumn{1}{c|}{{\color[HTML]{FE0000} 11.26}} & \multicolumn{1}{c|}{{\color[HTML]{FE0000} 10.44}} & {\color[HTML]{FE0000} 45} \\
                                    &                                                                                 & {\color[HTML]{FE0000} 100\% TL}              & {\color[HTML]{FE0000} 95.73} & {\color[HTML]{FE0000} 95.73} & {\color[HTML]{FE0000} 96.02} & {\color[HTML]{FE0000} 95.84} & {\color[HTML]{FE0000} 7.76}                 & \multicolumn{1}{c|}{{\color[HTML]{FE0000} 11.26}} & \multicolumn{1}{c|}{{\color[HTML]{FE0000} 10.44}} & {\color[HTML]{FE0000} 37} \\ \cline{3-11} 
                                    &                                                                                 & 10\% TL                                      & 93.53                        & 93.65                        & 93.93                        & 93.71                        & 4.29                                        & \multicolumn{1}{c|}{16.38}                        & \multicolumn{1}{c|}{10.77}                        & 90                        \\
                                    &                                                                                 & 50\% TL                                      & 97.25                        & 97.32                        & 97.27                        & 97.29                        & 8.64                                        & \multicolumn{1}{c|}{19.46}                        & \multicolumn{1}{c|}{10.77}                        & 89                        \\
                                    &                                                                                 & 80\% TL                                      & 97.83                        & 97.90                        & 97.82                        & 97.86                        & 12.77                                       & \multicolumn{1}{c|}{23.55}                        & \multicolumn{1}{c|}{10.44}                        & 92                        \\
\multirow{-24}{*}{Image}            & \multirow{-9}{*}{\begin{tabular}[c]{@{}c@{}}IMCFN
\end{tabular}} & 100\% TL                                     & \textbf{97.95}               & \textbf{98.03}               & \textbf{97.95}               & \textbf{97.98}               & 14.04                                       & \multicolumn{1}{c|}{25.60}                        & \multicolumn{1}{c|}{10.77}                        & 89                        \\ \hline
                                    & CBOW+MLP                                                                        & -                                            & \textbf{97.81}               & \textbf{97.92}               & \textbf{98.08}               & \textbf{98.00}               & 0.82                                        & \multicolumn{1}{c|}{51.94}                        & \multicolumn{1}{c|}{10.44}                        & 34                        \\
\multirow{-2}{*}{Binary}            & MalConv                                                                         & -                                            & 95.92                        & 96.04                        & 96.43                        & 96.20                        & 65.40                                       & \multicolumn{1}{c|}{246.78}                       & \multicolumn{1}{c|}{10.78}                        & 60                        \\ \hline
                                    & MAGIC                                                                           & -                                            & 92.82                        & 88.03                        & 87.36                        & 87.45                        & 246.00                                      & \multicolumn{1}{c|}{113.66}                       & \multicolumn{1}{c|}{10.61}                        & 81                        \\
                                    & Word2Vec+KNN                                                                    & -                                            & 95.64                        & 93.34                        & 94.29                        & 93.79                        & 0                                           & \multicolumn{1}{c|}{5.54}                         & \multicolumn{1}{c|}{-}                            & -                         \\
\multirow{-3}{*}{Disassembly}       & MCSC                                                                            & -                                            & \textbf{96.80}               & \textbf{94.97}               & \textbf{94.51}               & \textbf{94.70}               & 1.07                                        & \multicolumn{1}{c|}{45.34}                        & \multicolumn{1}{c|}{10.77}                        & 33                        \\ \hline
\bottomrule
\end{tabular}
\footnotesize
\yx{red data: IMCFN doesn't open the last feature extraction block (setting is consistent with other models). 
~\\
next black data: IMCFN open the last feature extraction block.
~\\
MalwareBazaar dataset is more balanced.}
\end{threeparttable}
\end{table*}
\end{comment}






\begin{comment}
\begin{table*}[t]
\centering\footnotesize
\begin{threeparttable}
\caption{Comparison of Classification Performance of Various Methods Based on 10-fold Cross-validation on the MalwareBazaar Dataset\jj{Transfer Learning can be shortened, such as TL to save space and for clarity.} \yx{Done.}}
\label{tab:MalwareBazaar-openextractlayer}
\begin{tabular}{c|c|c|cccc|c|ccc}
\toprule
\hline
\multirow{2}{*}{\textbf{Category}} & \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Training Strategy}} & \multicolumn{4}{c|}{\textbf{Classification Performance (\%)}}     & \multirow{2}{*}{\textbf{Train Time (min)}} & \multicolumn{3}{c}{\textbf{Resource Overhead}}                                                        \\ \cline{4-7} \cline{9-11} 
                                   &                                 &                                             & \textbf{A}     & \textbf{P}     & \textbf{R}     & \textbf{F1}    &                                            & \multicolumn{1}{c|}{\textbf{Mem (GB)}} & \multicolumn{1}{c|}{\textbf{G.Mem (MiB)}} & \textbf{GPU (\%)} \\ \hline
\multirow{20}{*}{Image}            & \multirow{5}{*}{ResNet-50}      & From Scratch                                & \textbf{96.68} & \textbf{96.91} & \textbf{96.75} & \textbf{96.83} & 8.35                                       & \multicolumn{1}{c|}{17.41}             & \multicolumn{1}{c|}{10.77}                & 95                \\
                                   &                                 & 10\% TL                                     & 90.03          & 89.48          & 90.99          & 90.09          & 4.07                                       & \multicolumn{1}{c|}{9.14}              & \multicolumn{1}{c|}{10.56}                & 6                 \\
                                   &                                 & 50\% TL                                     & 93.98          & 94.28          & 94.57          & 94.38          & 7.23                                       & \multicolumn{1}{c|}{9.13}              & \multicolumn{1}{c|}{10.56}                & 7                 \\
                                   &                                 & 80\% TL                                     & 94.90          & 95.21          & 95.34          & 95.25          & 9.11                                       & \multicolumn{1}{c|}{9.16}              & \multicolumn{1}{c|}{10.56}                & 5                 \\
                                   &                                 & 100\% TL                                    & 95.30          & 95.66          & 95.68          & 95.65          & 10.01                                      & \multicolumn{1}{c|}{9.19}              & \multicolumn{1}{c|}{10.56}                & 6                 \\ \cline{2-11} 
                                   & \multirow{5}{*}{VGG-16}         & From Scratch                                & \textbf{96.35} & \textbf{96.58} & \textbf{96.54} & \textbf{96.56} & 43.96                                      & \multicolumn{1}{c|}{18.43}             & \multicolumn{1}{c|}{10.77}                & 97                \\
                                   &                                 & 10\% TL                                     & 83.55          & 86.50          & 76.12          & 76.80          & 1.16                                       & \multicolumn{1}{c|}{8.17}              & \multicolumn{1}{c|}{10.44}                & 56                \\
                                   &                                 & 50\% TL                                     & 92.35          & 92.75          & 92.54          & 92.51          & 2.19                                       & \multicolumn{1}{c|}{9.34}              & \multicolumn{1}{c|}{10.44}                & 52                \\
                                   &                                 & 80\% TL                                     & 93.85          & 93.92          & 94.37          & 94.06          & 2.98                                       & \multicolumn{1}{c|}{10.24}             & \multicolumn{1}{c|}{10.44}                & 55                \\
                                   &                                 & 100\% TL                                    & 94.43          & 94.43          & 94.90          & 94.60          & 3.94                                       & \multicolumn{1}{c|}{11.26}             & \multicolumn{1}{c|}{10.44}                & 52                \\ \cline{2-11} 
                                   & \multirow{5}{*}{Inception-V3}   & From Scratch                                & \textbf{95.83} & \textbf{95.67} & \textbf{95.79} & \textbf{95.73} & 6.39                                       & \multicolumn{1}{c|}{12.29}             & \multicolumn{1}{c|}{10.77}                & 96                \\
                                   &                                 & 10\% TL                                     & 90.28          & 90.87          & 90.99          & 90.87          & 0.79                                       & \multicolumn{1}{c|}{7.83}              & \multicolumn{1}{c|}{10.56}                & 7                 \\
                                   &                                 & 50\% TL                                     & 93.75          & 94.31          & 94.20          & 94.24          & 3.77                                       & \multicolumn{1}{c|}{8.13}              & \multicolumn{1}{c|}{10.56}                & 8                 \\
                                   &                                 & 80\% TL                                     & 94.48          & 94.96          & 94.87          & 94.90          & 6.37                                       & \multicolumn{1}{c|}{8.70}              & \multicolumn{1}{c|}{10.56}                & 6                 \\
                                   &                                 & 100\% TL                                    & 94.80          & 95.15          & 95.17          & 95.15          & 8.47                                       & \multicolumn{1}{c|}{8.47}              & \multicolumn{1}{c|}{10.56}                & 7                 \\ \cline{2-11} 
                                   & \multirow{5}{*}{IMCFN}          & From Scratch                                & 97.38          & 97.53          & 97.41          & 97.47          & 18.75                                      & \multicolumn{1}{c|}{22.53}             & \multicolumn{1}{c|}{10.77}                & 92                \\
                                   &                                 & 10\% TL                                     & 93.53          & 93.65          & 93.93          & 93.71          & 4.29                                       & \multicolumn{1}{c|}{16.38}             & \multicolumn{1}{c|}{10.77}                & 90                \\
                                   &                                 & 50\% TL                                     & 97.25          & 97.32          & 97.27          & 97.29          & 8.64                                       & \multicolumn{1}{c|}{19.46}             & \multicolumn{1}{c|}{10.77}                & 89                \\
                                   &                                 & 80\% TL                                     & 97.83          & 97.90          & 97.82          & 97.86          & 12.77                                      & \multicolumn{1}{c|}{23.55}             & \multicolumn{1}{c|}{10.44}                & 92                \\
                                   &                                 & 100\% TL                                    & \textbf{97.95} & \textbf{98.03} & \textbf{97.95} & \textbf{97.98 (\yx{96.71$^\star$})} & 14.04                                      & \multicolumn{1}{c|}{25.60}             & \multicolumn{1}{c|}{10.77}                & 89                \\ \hline
\multirow{2}{*}{Binary}            & CBOW+MLP                        & -                                           & \textbf{97.81} & \textbf{97.92} & \textbf{98.08} & \textbf{98.00} & 0.82                                       & \multicolumn{1}{c|}{51.94}             & \multicolumn{1}{c|}{10.44}                & 34                \\
                                   & MalConv                         & -                                           & 95.92          & 96.04          & 96.43          & 96.20          & 65.40                                      & \multicolumn{1}{c|}{246.78}            & \multicolumn{1}{c|}{10.78}                & 60                \\ \hline
\multirow{3}{*}{Disassembly}       & MAGIC                           & -                                           & 92.82          & 88.03          & 87.36          & 87.45          & 246.00                                     & \multicolumn{1}{c|}{113.66}            & \multicolumn{1}{c|}{10.61}                & 81                \\
                                   & Word2Vec+KNN                    & -                                           & 95.64          & 93.34          & 94.29          & 93.79          & $\approx{0}$                                          & \multicolumn{1}{c|}{5.54}              & \multicolumn{1}{c|}{-}                    & -                 \\
                                   & MCSC                            & -                                           & \textbf{96.80} & \textbf{94.97} & \textbf{94.51} & \textbf{94.70} & 1.07                                       & \multicolumn{1}{c|}{45.34}             & \multicolumn{1}{c|}{10.77}                & 33                \\ \hline
\bottomrule
\end{tabular}
\footnotesize
\yx{red data: IMCFN doesn't open the last feature extraction block (setting is consistent with other models).
~\\
MalwareBazaar dataset is more balanced.}
\end{threeparttable}
\end{table*}
\end{comment}








\begin{comment}
\begin{table*}[t]
\centering\scriptsize
\begin{threeparttable}
\caption{Comparison of Classification Performance of Various Methods Based on 10-fold Cross-validation on the MalwareBazaar Dataset\jj{Transfer Learning can be shortened, such as TL to save space and for clarity.}}
\label{tab:Compare-MalwareBazaar-no reasource comsume}
\begin{tabular}{c|c|c|cccc|c|c|lll}
\toprule
\hline
\multirow{2}{*}{\textbf{Category}} & \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Training Strategy}} & \multicolumn{4}{c|}{\textbf{Classification Performance (\%)}}     & \multicolumn{2}{c|}{\textbf{Time}}            & \multicolumn{3}{c}{\textbf{Reasource Overhead}}                                                                        \\ \cline{4-12} 
                                   &                                 &                                             & \textbf{A}     & \textbf{P}     & \textbf{R}     & \textbf{F1}    & \textbf{Pre (s)}       & \textbf{Train (min)} & \multicolumn{1}{c|}{\textbf{V.Mem (GB)}} & \multicolumn{1}{c|}{\textbf{G.Mem (GB)}} & \multicolumn{1}{c}{\textbf{GPU}} \\ \hline
\multirow{20}{*}{Image}            & \multirow{5}{*}{ResNet-50}      & From Scratch                                & \textbf{96.68} & \textbf{96.91} & \textbf{96.75} & \textbf{96.83} & \multirow{20}{*}{0.70} & 8.35                 & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\
                                   &                                 & 10\%-Transfer                               & 90.03          & 89.48          & 90.99          & 90.09          &                        & 4.07                 & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\
                                   &                                 & 50\%-Transfer                               & 93.98          & 94.28          & 94.57          & 94.38          &                        & 7.23                 & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\
                                   &                                 & 80\%-Transfer                               & 94.90          & 95.21          & 95.34          & 95.25          &                        & 9.11                 & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\
                                   &                                 & 100\%-Transfer                              & 95.30          & 95.66          & 95.68          & 95.65          &                        & 10.01                & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\ \cline{2-7} \cline{9-12} 
                                   & \multirow{5}{*}{VGG-16}         & From Scratch                                & \textbf{96.35} & \textbf{96.58} & \textbf{96.54} & \textbf{96.56} &                        & 43.96                & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\
                                   &                                 & 10\%-Transfer                               & 83.55          & 86.50          & 76.12          & 76.80          &                        & 1.16                 & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\
                                   &                                 & 50\%-Transfer                               & 92.35          & 92.75          & 92.54          & 92.51          &                        & 2.19                 & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\
                                   &                                 & 80\%-Transfer                               & 93.85          & 93.92          & 94.37          & 94.06          &                        & 2.98                 & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\
                                   &                                 & 100\%-Transfer                              & 94.43          & 94.43          & 94.90          & 94.60          &                        & 3.94                 & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\ \cline{2-7} \cline{9-12} 
                                   & \multirow{5}{*}{Inception-V3}   & From Scratch                                & \textbf{95.83} & \textbf{95.67} & \textbf{95.79} & \textbf{95.73} &                        & 6.39                 & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\
                                   &                                 & 10\%-Transfer                               & 90.28          & 90.87          & 90.99          & 90.87          &                        & 0.79                 & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\
                                   &                                 & 50\%-Transfer                               & 93.75          & 94.31          & 94.20          & 94.24          &                        & 3.77                 & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\
                                   &                                 & 80\%-Transfer                               & 94.48          & 94.96          & 94.87          & 94.90          &                        & 6.37                 & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\
                                   &                                 & 100\%-Transfer                              & 94.80          & 95.15          & 95.17          & 95.15          &                        & 8.47                 & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\ \cline{2-7} \cline{9-12} 
                                   & \multirow{5}{*}{IMCFN}          & From Scratch                                & 97.38          & 97.53          & 97.41          & 97.47          &                        & 18.75                & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\
                                   &                                 & 10\%-Transfer                               & 93.53          & 93.65          & 93.93          & 93.71          &                        & 4.29                 & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\
                                   &                                 & 50\%-Transfer                               & 97.25          & 97.32          & 97.27          & 97.29          &                        & 8.64                 & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\
                                   &                                 & 80\%-Transfer                               & 97.83          & 97.90          & 97.82          & 97.86          &                        & 12.77                & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\
                                   &                                 & 100\%-Transfer                              & \textbf{97.95} & \textbf{98.03} & \textbf{97.95} & \textbf{97.98} &                        & 14.04                & \multicolumn{1}{c|}{64.14}               & \multicolumn{1}{c|}{10.77}               & \multicolumn{1}{c}{90\%}         \\ \hline
\multirow{2}{*}{Binary}            & CBOW+MLP                        & -                                           & 97.81          & 97.92          & \textbf{98.08} & \textbf{98.00} & 6.52                   & 0.82                 & \multicolumn{1}{c|}{51.94}               & \multicolumn{1}{c|}{10.44}               & \multicolumn{1}{c}{34\%}         \\
                                   & MalConv                         & -                                           & 95.92          & 96.04          & 96.43          & 96.20          & 0.10                   & 65.40                & \multicolumn{1}{c|}{246.78}              & \multicolumn{1}{c|}{10.78}               & \multicolumn{1}{c}{60\%}         \\ \hline
\multirow{3}{*}{Disassembly}       & MAGIC                           & -                                           & 92.82          & 88.03          & 87.36          & 87.45          & 18.42                  & 246.00               & \multicolumn{1}{c|}{113.66}              & \multicolumn{1}{c|}{10.61}               & \multicolumn{1}{c}{81\%}         \\
                                   & Word2Vec+KNN                    & -                                           & 95.64          & 93.34          & 94.29          & 93.79          & 13.58                  & -                    & \multicolumn{1}{c|}{5.54}                & \multicolumn{1}{c|}{-}                   & \multicolumn{1}{c}{-}            \\
                                   & MCSC                            & -                                           & 96.80          & 94.97          & 94.51          & 94.70          & 5.34                   & 1.07                 & \multicolumn{1}{c|}{45.34}               & \multicolumn{1}{c|}{10.77}               & \multicolumn{1}{c}{33\%}         \\ \hline
\bottomrule
\end{tabular}
\end{threeparttable}
\end{table*}
\end{comment}











\begin{comment}
\begin{table*}[t]
\centering\scriptsize
\begin{threeparttable}
\caption{Comparison of Classification Performance of Various Methods Based on 10-fold Cross-validation on the MalwareBazaar Dataset\jj{Transfer Learning can be shortened, such as TL to save space and for clarity.}}
\label{tab:Compare-MalwareBazaar-incomplete-version}
\begin{tabular}{l|c|c|cccc|c|c|lll}
\toprule
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Category}}} & \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Training Strategy}}  & \multicolumn{4}{c|}{\textbf{Classification Performance (\%)}} & \multicolumn{2}{c|}{\textbf{Time}}      & \multicolumn{3}{c}{\textbf{Reasource Overhead}}                                                                        \\ \cline{4-12} 
\multicolumn{1}{c|}{}                                   &                                 &                                              & \textbf{A}    & \textbf{P}    & \textbf{R}    & \textbf{F1}   & \textbf{Pre (s)} & \textbf{Train (min)} & \multicolumn{1}{c|}{\textbf{V.Mem (GB)}} & \multicolumn{1}{c|}{\textbf{G.Mem (GB)}} & \multicolumn{1}{c}{\textbf{GPU}} \\ \hline
\multirow{20}{*}{Image}                                 & \multirow{5}{*}{ResNet-50}      & Train From Scretch                           & 96.68         & 96.91         & 96.75         & 96.83         &                  & 8.35                 & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\
                                                        &                                 & 10\%-Transfer Learning                       &               & \textbf{}     &               & \textbf{}     &                  &                      & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\
                                                        &                                 & 50\%-Transfer Learning                       &               &               &               &               & \textbf{}        & \textbf{}            & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\
                                                        &                                 & 80\%-Transfer Learning                       &               &               &               &               &                  &                      & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\
                                                        &                                 & \multicolumn{1}{l|}{100\%-Transfer Learning} &               &               &               &               &                  &                      & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\ \cline{2-7} \cline{9-12} 
                                                        & \multirow{5}{*}{VGG-16}         & Train From Scretch                           & 96.35         & 96.58         & 96.54         & 96.56         &                  & 43.96                & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\
                                                        &                                 & 10\%-Transfer Learning                       &               &               &               &               & \textbf{}        & \textbf{}            & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\
                                                        &                                 & 50\%-Transfer Learning                       &               &               &               &               & \textbf{}        & \textbf{}            & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\
                                                        &                                 & 80\%-Transfer Learning                       & \textbf{}     &               & \textbf{}     &               & \textbf{}        & \textbf{}            & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\
                                                        &                                 & \multicolumn{1}{l|}{100\%-Transfer Learning} & 94.43         & 94.43         & 94.90         & 94.60         &                  & 3.94                 & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\ \cline{2-7}
                                                        & \multirow{5}{*}{Inception-V3}   & Train From Scretch                           & 95.83         & 95.67         & 95.79         & 95.73         &                  & 6.39                 & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\
                                                        &                                 & 10\%-Transfer Learning                       &               &               & \textbf{}     &               &                  &                      & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\
                                                        &                                 & 50\%-Transfer Learning                       & \textbf{}     & \textbf{}     & \textbf{}     & \textbf{}     &                  &                      & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\
                                                        &                                 & 80\%-Transfer Learning                       &               &               & \textbf{}     &               &                  &                      & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\
                                                        &                                 & \multicolumn{1}{l|}{100\%-Transfer Learning} &               &               &               &               & \textbf{}        & \textbf{}            & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\ \cline{2-7}
                                                        & \multirow{5}{*}{IMCFN}          & Train From Scretch                           & 97.38         & 97.53         & 97.41         & 97.47         &                  & 18.75                & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\
                                                        &                                 & 10\%-Transfer Learning                       & \textbf{}     & \textbf{}     & \textbf{}     & \textbf{}     &                  &                      & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\
                                                        &                                 & 50\%-Transfer Learning                       & \textbf{}     & \textbf{}     &               & \textbf{}     &                  &                      & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\
                                                        &                                 & 80\%-Transfer Learning                       & \textbf{}     & \textbf{}     &               & \textbf{}     & \textbf{}        & \textbf{}            & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}                    &                                  \\
                                                        &                                 & \multicolumn{1}{l|}{100\%-Transfer Learning} & 98.13         & 98.39         & 98.10         & 98.24         & 0.70             & 63.15                & \multicolumn{1}{c|}{102.40}              & \multicolumn{1}{c|}{10.77}               & \multicolumn{1}{c}{90\%}         \\ \cline{1-7} \cline{9-12} 
\multicolumn{1}{c|}{\multirow{2}{*}{Binary}}            & CBOW+MLP                        & -                                            & 97.81         & 97.92         & 98.08         & 98.00         & 6.52             & 0.82                 & \multicolumn{1}{c|}{51.94}               & \multicolumn{1}{c|}{10.44}               & \multicolumn{1}{c}{34\%}         \\
\multicolumn{1}{c|}{}                                   & MalConv                         & -                                            & 95.92         & 96.04         & 96.43         & 96.20         & 0.10             & 65.40                & \multicolumn{1}{c|}{246.78}              & \multicolumn{1}{c|}{10.78}               & \multicolumn{1}{c}{60\%}         \\ \hline
\multicolumn{1}{c|}{\multirow{3}{*}{Disassembly}}       & MAGIC                           & -                                            & 92.82         & 88.03         & 87.36         & 87.45         & 18.42            & 246.00               & \multicolumn{1}{c|}{113.66}              & \multicolumn{1}{c|}{10.61}               & \multicolumn{1}{c}{81\%}         \\
\multicolumn{1}{c|}{}                                   & Word2Vec+k-NN                   & -                                            & 95.64         & 93.34         & 94.29         & 93.79         & 13.58            & -                    & \multicolumn{1}{c|}{5.54}                & \multicolumn{1}{c|}{-}                   & \multicolumn{1}{c}{-}            \\
\multicolumn{1}{c|}{}                                   & MCSC                            & -                                            & 96.80         & 94.97         & 94.51         & 94.70         & 5.34             & 1.07                 & \multicolumn{1}{c|}{45.34}               & \multicolumn{1}{c|}{10.77}               & \multicolumn{1}{c}{33\%}         \\ \hline
\bottomrule
\end{tabular}
\end{threeparttable}
\end{table*}
\end{comment}































\begin{comment}
\begin{table*}[t]
\centering
\begin{threeparttable}
\caption{Comparison of Classification Performance of Various Methods Based on 10-fold Cross-validation on the MalwareBazaar Dataset}
\label{tab:Compare-malwarebazaar-Non-uniform calculation criteria}
\footnotesize
\begin{tabular}{ccccccccccc}
\toprule
\hline
\multirow{2}{*}{Category}    & \multirow{2}{*}{Method} & \multicolumn{4}{c}{Average Classification Performance (\%)} & \multicolumn{3}{c}{Resource Overhead}        & \multicolumn{2}{c}{Time (min)} \\
                             &                         & A             & P             & R            & F1           & V.Mem (GB) & G.Mem (GB) & GPU  & Pre-process (s)    & Train (min)   \\ \hline
Image                        & IMCFN                   & 98.13         & 98.41         & 98.10        & 98.24        & 102.40              & 11.30           & 90\% & 0.70           & 63.15         \\ \hline
\multirow{2}{*}{Binary}      & CBOW+MLP                & 97.81         & 97.94         & 98.08        & 98.00        & 51.94               & 10.95           & 34\% & 6.52           & 0.82          \\
                             & MalConv                 & 95.91         & 96.15         & 96.42        & 96.21        & 246.78              & 11.30           & 60\% & 0.10           & 65.40         \\ \hline
\multirow{3}{*}{Disassembly} & MAGIC                   & 92.83         & 88.93         & 87.30        & 86.10        & 68.74      113.66   & 11.13           & 81\% & 18.42        & 246.00        \\
                             & Word2Vec+KNN           & 95.65         & 93.96         & 94.31        & 93.80        & 5.54        0.33    & -               & -    & 13.58 (4.44)          & -             \\
                             & MCSC(Simhash)           & 96.80         & 95.66         & 94.75        & 94.77        & 45.34               & 11.30           & 33\% & 5.34           & 1.07          \\ \hline

\bottomrule
\end{tabular}
\footnotesize
  Note:  
%\begin{tablenotes}
%  \item[*] 
%  \item[**] 
%\end{tablenotes}
\end{threeparttable}
\end{table*}
\end{comment}


\begin{comment}
\begin{table*}[t]
\centering
\begin{threeparttable}
\caption{Comparison of Classification Performance of Various Methods  on the MalwareBazaar Dataset\jj{Duplicate? Pls comment out either Table VII or Table VIII.}}
\label{tab:Compare-malwarebazaar-Uniform computing standard}
\footnotesize
\begin{tabular}{ccccccccccc}
\toprule
\hline
\multirow{2}{*}{Catefory}    & \multirow{2}{*}{Method} & \multicolumn{4}{c}{Average Classification Performance (\%)}       & \multicolumn{3}{c}{Resource Overhead} & \multicolumn{2}{c}{Time}      \\
                             &                         & A              & P              & R              & F1             & V.Mem (GB)     & G.Mem (GB)   & GPU   & Pre-process (s) & Train (min) \\ \hline
Image                        & IMCFN                   & \textbf{98.13} & \textbf{98.39} & \textbf{98.10} & \textbf{98.24} & 102.40         & 11.30        & 90\%  & 0.70            & 63.15       \\ \hline
\multirow{2}{*}{Binary}      & CBOW+MLP                & 97.81          & 97.92          & 98.08          & 98.00          & 51.94          & 10.95        & 34\%  & 6.52            & 0.82        \\
                             & MalConv                 & 95.92          & 96.04          & 96.43          & 96.20          & 246.78         & 11.30        & 60\%  & 0.10            & 65.40       \\ \hline
\multirow{3}{*}{Disassembly} & DGCNN                   & 92.82          & 88.03          & 87.36          & 87.45          & 113.66         & 11.13        & 81\%  & 18.42           & 246.00      \\
                             & Word2Vec+KNN           & 95.64          & 93.34          & 94.29          & 93.79          & 5.54    0.33   & -            & -     & 13.58 (4.44)    & -           \\
                             & MCSC(Simhash)           & 96.80          & 94.97          & 94.51          & 94.70          & 45.34          & 11.30        & 33\%  & 5.34            & 1.07        \\ \hline
\bottomrule
\end{tabular}
\footnotesize
\end{threeparttable}
\end{table*}
\end{comment}

==> tab_result_transfer.tex <==
\begin{table*}[t]
\centering
\tiny
\begin{threeparttable}
\caption{Results of image-based classification techniques on BIG-15 and Malimg Dataset}
\label{tab:image-based-result}
\begin{tabular}{lc|cccc|c|cccc|c|ccccc}
\toprule

\hline
\multirow{3}{*}{\textbf{Training Strategy}}                                                            & \multirow{3}{*}{\textbf{Model Architecture}} & \multicolumn{5}{c|}{\textbf{BIG-15 Dataset}}                                              & \multicolumn{5}{c|}{\textbf{Malimg Dataset}}                                              & \multicolumn{5}{c}{\textbf{MalwareBazaar Dataset}}                                                                                                                              \\ \cline{3-17} 
                                                                                                       &                                              & \multicolumn{4}{c|}{\textbf{Macro Average (\%)}}                  & \textbf{Time (min)}   & \multicolumn{4}{c|}{\textbf{Macro Average (\%)}}                  & \textbf{Time (min)}   & \multicolumn{4}{c}{\textbf{Macro Average (\%)}}                                                                                     & \multicolumn{1}{l}{\textbf{Time (min)}}   \\ \cline{3-17} 
                                                                                                       &                                              & \textbf{A}     & \textbf{P}     & \textbf{R}     & \textbf{F1}    & \textbf{Train / fold} & \textbf{A}     & \textbf{P}     & \textbf{R}     & \textbf{F1}    & \textbf{Train / fold} & \multicolumn{1}{l}{\textbf{A}} & \multicolumn{1}{l}{\textbf{P}} & \multicolumn{1}{l}{\textbf{R}} & \multicolumn{1}{l|}{\textbf{F1}} & \multicolumn{1}{l}{\textbf{Train / fold}} \\ \hline
\multirow{4}{*}{\textbf{Train From Scretch}}                                                           & ResNet-50                                    & \textbf{98.42} & \textbf{96.57} & \textbf{95.68} & \textbf{96.08} & 203.70                & 98.14          & 95.48          & 95.06          & 95.21          & 175.02                & 96.68                          & 96.91                          & 96.75                          & \multicolumn{1}{c|}{96.83}       & 8.35                                      \\
                                                                                                       & VGG-16                                       & 93.94          & 90.32          & 81.89          & 87.28          & 275.52                & 99.08          & 97.71          & \textbf{97.74} & 97.73          & 94.56                 & 96.35                          & 96.58                          & 96.54                          & \multicolumn{1}{c|}{96.56}       & 43.96                                     \\
                                                                                                       & Inception-V3                                 & 96.99          & 93.67          & 94.46          & 94.03          & \textbf{150.00}       & 97.77          & 96.29          & 93.82          & 93.98          & 273.12                & 95.83                          & 95.67                          & 95.79                          & \multicolumn{1}{c|}{95.73}       & 6.39                                      \\
                                                                                                       & IMCFN                                        & 97.70          & 95.49          & 93.70          & 94.44          & 277.08                & \textbf{99.13} & \textbf{98.08} & 97.62          & \textbf{97.84} & \textbf{79.44}        & 97.38                          & 97.53                          & 97.41                          & \multicolumn{1}{c|}{97.47}       & 18.75                                     \\ \hline
\multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Transfer Learning\\ 10\%-Train Data\end{tabular}}}  & ResNet-50                                    & 94.76          & \textbf{92.74} & 82.69          & \textbf{86.77} & 8.58                  & \textbf{97.34} & 93.79          & \textbf{92.77} & \textbf{93.21} & 15.12                 &                                &                                &                                & \multicolumn{1}{c|}{}            &                                           \\
                                                                                                       & VGG-16                                       & 89.56          & 78.74          & 76.73          & 77.59          & \textbf{1.52}         & 96.37          & 90.05          & 89.24          & 89.50          & \textbf{2.40}         &                                &                                &                                & \multicolumn{1}{c|}{}            &                                           \\
                                                                                                       & Inception-V3                                 & 92.28          & 91.46          & 80.51          & 80.94          & 4.44                  & 93.82          & 87.07          & 83.93          & 85.05          & 3.93                  &                                &                                &                                & \multicolumn{1}{c|}{}            &                                           \\
                                                                                                       & IMCFN                                        & \textbf{94.80} & 89.05          & \textbf{82.76} & 83.77          & 18.18                 & 97.19          & \textbf{94.41} & 91.82          & 92.60          & 26.34                 &                                &                                &                                & \multicolumn{1}{c|}{}            &                                           \\ \hline
\multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Transfer Learning\\ 50\%-Train Data\end{tabular}}}  & ResNet-50                                    & 96.68          & 95.35          & 85.22          & 91.50          & 24.78                 & 98.02          & 95.61          & 94.46          & 94.93          & 42.30                 &                                &                                &                                & \multicolumn{1}{c|}{}            &                                           \\
                                                                                                       & VGG-16                                       & 95.21          & 89.02          & 83.77          & 87.21          & \textbf{11.76}        & 97.24          & 91.29          & 91.64          & 91.41          & \textbf{7.32}         &                                &                                &                                & \multicolumn{1}{c|}{}            &                                           \\
                                                                                                       & Inception-V3                                 & 95.10          & 91.17          & \textbf{86.76} & 86.87          & 12.78                 & 95.75          & 89.23          & 88.63          & 88.86          & 11.04                 &                                &                                &                                & \multicolumn{1}{c|}{}            &                                           \\
                                                                                                       & IMCFN                                        & \textbf{97.93} & \textbf{95.43} & 86.67          & \textbf{93.64} & 53.94                 & \textbf{98.64} & \textbf{96.41} & \textbf{96.35} & \textbf{96.37} & 79.80                 &                                &                                &                                & \multicolumn{1}{c|}{}            &                                           \\ \hline
\multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Transfer Learning\\ 80\%-Train Data\end{tabular}}}  & ResNet-50                                    & 96.90          & 94.87          & 85.53          & 92.50          & 37.02                 & 98.59          & 96.37          & 96.23          & 96.29          & 63.78                 & 95.30                          & 95.71                          & 95.65                          & \multicolumn{1}{c|}{95.66}       & 14.40                                     \\
                                                                                                       & VGG-16                                       & 96.62          & 92.00          & 85.20          & 90.41          & \textbf{8.04}         & 98.58          & 96.35          & 96.23          & 96.28          & \textbf{11.46}        &                                &                                &                                & \multicolumn{1}{c|}{}            &                                           \\
                                                                                                       & Inception-V3                                 & 95.31          & 92.52          & \textbf{88.54} & 88.64          & 19.02                 & 96.17          & 90.15          & 89.61          & 89.84          & 16.32                 &                                &                                &                                & \multicolumn{1}{c|}{}            &                                           \\
                                                                                                       & IMCFN                                        & \textbf{98.48} & \textbf{96.90} & 87.31          & \textbf{95.38} & 134.34                & \textbf{99.00} & \textbf{97.42} & \textbf{97.40} & \textbf{97.41} & 117.66                &                                &                                &                                & \multicolumn{1}{c|}{}            &                                           \\ \hline
\multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Transfer Learning\\ 100\%-Train Data\end{tabular}}} & ResNet-50                                    & 97.05          & 95.64          & 93.60          & 94.48          & 43.62                 & 98.49          & 96.33          & 95.88          & 96.10          & 70.80                 & 95.30                          & 95.66                          & 95.68                          & \multicolumn{1}{c|}{95.65}       & 11.99                                     \\
                                                                                                       & VGG-16                                       & 96.78          & 93.36          & 91.78          & 92.46          & \textbf{9.72}         & 98.63          & 96.47          & 96.40          & 96.42          & \textbf{14.16}        & 94.43                          & 94.43                          & 94.90                          & \multicolumn{1}{c|}{94.60}       & 3.94                                      \\
                                                                                                       & Inception-V3                                 & 95.56          & 93.48          & 89.64          & 89.76          & 22.92                 & 96.43          & 90.62          & 90.28          & 90.41          & 18.96                 & 94.50                          & 95.00                          & 94.85                          & \multicolumn{1}{c|}{94.92}       & 10.55                                     \\
                                                                                                       & IMCFN                                        & \textbf{99.17} & \textbf{98.69} & \textbf{97.52} & \textbf{98.07} & 166.68                & \textbf{99.08} & \textbf{97.62} & \textbf{97.57} & \textbf{97.59} & 146.94                & 98.13                          & 98.39                          & 98.10                          & \multicolumn{1}{c|}{98.24}       & 63.15                                     \\ \hline

\bottomrule
\end{tabular}
\small
\textbf{A}, \textbf{P}, \textbf{R} and \textbf{F1} represent the macro average of accuracy, precision, recall and F1-score on the test set, respectively. The training time for each model on one fold is reported. We report the results of 5 training strategies, one for normal supervised training and the other 4 for transfer learning with different dataset size of the target domain. The best results are highlighted in bold. 
\end{threeparttable}
\end{table*}

==> tab_settings.tex <==
\begin{comment}
\begin{table}[t]
\centering
\begin{threeparttable}
\caption{Model Parameters}
\label{tab:image-based-model-parameters}
\begin{tabular}{c|cc}
\toprule
\hline
\multirow{2}{*}{Model} & \multicolumn{2}{c}{Parameters}                                         \\ \cline{2-3} 
                       & \multicolumn{1}{c|}{Feature Extraction Layers} & Classification Layers \\ \hline
ResNet-50              & \multicolumn{1}{c|}{23,587,712}                & 18,441                \\
VGG-16                 & \multicolumn{1}{c|}{14,714,688}                & 119,582,729           \\
Inception-V3           & \multicolumn{1}{c|}{21,802,784}                & 18,441                \\
IMCFN                  & \multicolumn{1}{c|}{14,714,688}                & 55,597,065            \\ \hline
\bottomrule
\end{tabular}
\end{threeparttable}
\end{table}
\end{comment}





\begin{table*}[t]
\centering
\small
\begin{threeparttable}
\caption{Hyper-parameter Settings  %\yx{Updated}
%\jj{This table seems not complete?} \yx{Done.}
}
\label{tab:setting}
\begin{tabular}{c|c|c|ccc|c}
\toprule
\hline
\multirow{2}{*}{Category}    & \multirow{2}{*}{Model}        & \multirow{2}{*}{Training Strategy} & \multicolumn{3}{c|}{Hyper-parameter}   & \multirow{2}{*}{Input Format}                                                                  \\ \cline{4-6}
                             &                               &                                    & Optimizer & Learning Rate & Batch Size &                                                                                                \\ \hline
\multirow{8}{*}{Image}       & \multirow{2}{*}{ResNet-50}    & From Scratch                       & Adam      & 1e-3             & 64         & \multirow{8}{*}{224*224 color image}                                                           \\ \cline{3-6}
                             &                               & Transfer                           & Adam      & 1e-3             & All data*  &                                                                                                \\ \cline{2-6}
                             & \multirow{2}{*}{VGG-16}       & From Scratch                       & SGD       & 5e-6**        & 64         &                                                                                                \\ \cline{3-6}
                             &                               & Transfer                           & SGD       & 5e-6          & 64         &                                                                                                \\ \cline{2-6}
                             & \multirow{2}{*}{Inception-V3} & From Scratch                       & Adam      & 1e-3             & 64         &                                                                                                \\ \cline{3-6}
                             &                               & Transfer                           & Adam      & 1e-3             & All data   &                                                                                                \\ \cline{2-6}
                             & \multirow{2}{*}{IMCFN}        & From Scratch                       & SGD       & 5e-6***       & 32         &                                                                                                \\ \cline{3-6}
                             &                               & Transfer                           & SGD       & 5e-6***      & 32         &                                                                                                \\ \hline
\multirow{2}{*}{Binary}      & CBOW+MLP                & -                                  & SGD       & 1e-3          & 128        & \begin{tabular}[c]{@{}c@{}}CBOW: byte sequences\\ MLP: 256*256 matrix\end{tabular}             \\ \cline{2-7} 
                             & MalConv                       & -                                  & SGD       & 1e-3          & 32         & 2MB raw byte values                                                                            \\ \hline
\multirow{3}{*}{Disassembly} & MAGIC                         & -                                  & Adam         & 1e-4             & 10         & ACFG                                                                                          \\ \cline{2-7} 
                             & Word2Vec+KNN            & -                                  & -         & -             & -          & \begin{tabular}[c]{@{}c@{}}Word2Vec: Opcode sequences\\ KNN distance measure: WMD\end{tabular} \\ \cline{2-7} 
                             & MCSC                          & -                                  & SGD       & 5e-3          & 64         & Opcode sequences                                                                           \\ \hline
\bottomrule
\end{tabular}
\footnotesize
\begin{tablenotes}
 \item[*] The batch size is set to 128 for the MalwareBazaar dataset
 \item[**] The learning rate is set to 5e-5 for the Malimg dataset and 1e-5 for the MalwareBazaar dataset 
 \item[***] The learning rate is set to 1e-5 for the MalwareBazaar dataset
 \item CBOW is with default parameters in the Word2Vec package in the Gensim library 
 %\item[*****] CBOW with default parameters in the Word2Vec package in Gensim library
 %\item[******] use CBOW model here with the window size = 5 and k = 1 in KNN
\end{tablenotes}
\end{threeparttable}
\vspace{-4mm}
\end{table*}
